Polynomial in Non-Commutative Algebra

I considered definition and properties of polynomial in no-commutative algebra. There exists polynomial which has finite, infinite or empty set of roots. For instance, the polynomial $$p_1(x)=ix-xi-1$$ have no root and the polynomial $$p_k(x)=ix-xi-k$$ has the set of roots $$x=C_1+C_2i+\frac 12 j$$ I considered division of polynomials with remainder.

==> Abstract.Monomial.English.tex <==
%auto-ignore

\AddEq[2]{remark: ix-xi-1 roots}
{
the polynomial
\DrawEq[1]{ix-xi-1}{#1}
have no root
and the polynomial
\DrawEq[k]{ix-xi-1}{#2}
has the set of roots
\DrawEq{x=c12+j}{#2}
}

\begin{abstract}
I considered definition and properties of polynomial
in non\Hyph commutative algebra.
There exists polynomial which has finite, infinite
or empty set of roots.
For instance,
\ShowRemark{ix-xi-1 roots}{}{}
I considered division of polynomials with remainder.
\end{abstract}


==> Abstract.Monomial.Russian.tex <==
%auto-ignore

\AddEq[2]{remark: ix-xi-1 roots}
{
многочлен
\DrawEq[1]{ix-xi-1}{#1}
не имеет корней
и многочлен
\DrawEq[k]{ix-xi-1}{#2}
имеет множество корней
\DrawEq{x=c12+j}{#2}
}

\begin{abstract}
Я рассмотрел определение и свойства многочлена
в некоммутативной алгебре.
Многочлен может иметь конечное или бесконечное,
а также пустое множество корней.
Например,
\ShowRemark{ix-xi-1 roots}{}{}
Рассмотрена операция деления многочленов с остатком.
\end{abstract}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}{\ShowCiteBib{0812.4763}}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}{\ShowCiteBib{1302.7204}}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1502.04063}{\ShowCiteBib{1502.04063}}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\BiblioItem{1601.03259}{\ShowCiteBib{1601.03259}}%

\BiblioItem{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}%

\BiblioItem{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2020.06.01}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.Russian.pdf)}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Александр Клейн,
Математический анализ над алгеброй кватернионов,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\BiblioItem{MVector}
{
Александр Клейн,
Линейное отображение D-алгебры,\\
eprint \href{http://arxiv.org/abs/MVector}{arXiv:MVector} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{0767-8264}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй: Экспонента,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\BiblioItem{1812.03397}{\ShowCiteBib{1812.03397}}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{1510.02224}{\ShowCiteBib{1510.02224}}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem{Cohn: Skew Fields}{\ShowCiteBib{Cohn: Skew Fields}}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{\ShowCiteBib{Sudbery Quaternionic Analysis}}

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%719%A%A столбец
   {$A$\Hyph столбец}%
   {A column}%
\Index%132%A%A строка
   {$A$\Hyph строка}%
   {A row}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%15%A%A-векторное пространство
   {$A$\hyph векторное пространство}%
   {A vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%134%C%cr-обратная матрица
   {\CR обратная матрица}%
   {cr-inverse matrix}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%218%R%rc-обратная матрица
   {\RC обратная матрица}%
   {rc-inverse matrix}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%959%Г%гомоморфизм векторного пространства
   {гомоморфизм векторного пространства}%
   {homomorphism of vector space}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%964%З%закон коммутативности
   {закон коммутативности}%
   {commutative law}%
\Index%701%З%закон сокращения
   {закон сокращения}%
   {cancellation law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%976%И%интегрируемая дифференциальная форма
   {интегрируемая дифференциальная форма}%
   {integrable differential form}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%368%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%913%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%535%К%квазибазис
   {квазибазис}%
   {quasibasis}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%258%К%колинеарные векторы
   {колинеарные векторы}%
   {colinear vectors}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация столбцов
   {левая линейная комбинация столбцов}%
   {left linear combination of columns}%
\Index%954%Л%левая линейная комбинация строк
   {левая линейная комбинация строк}%
   {left linear combination of rows}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%973%Л%левый смежный класс
   {левый смежный класс}%
   {left coset}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%136%Л%линейно зависимы слева
   {линейно зависимы слева}%
   {left linear dependent}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%255%М%матрица Вронского
   {матрица Вронского}%
   {Wronskian matrix}%
\Index%958%М%матрица гомоморфизма
   {матрица гомоморфизма}%
   {matrix of homomorphism}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%219%Н%невырожденная система правых AU* линейных уравнений
   {невырожденная система правых $A^*$\Hyph линейных уравнений}%
   {nonsingular system of right AU* linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%960%Н%непрерывный базис Шаудера
   {непрерывный базис Шаудера}%
   {continuous Schauder basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%702%Н%нормальная подгруппа
   {нормальная подгруппа}%
   {normal subgroup}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%970%О%образ отображения
   {образ отображения}%
   {image of map}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен
   {однородный многочлен}%
   {homogeneous polynomial}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%212%О%определитель Вронского
   {определитель Вронского}%
   {Wronskian determinant}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное G-представление
   {пассивное $G$\Hyph представление}%
   {passive G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation, vector space}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%963%П%первый интеграл
   {первый интеграл}%
   {first integral}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация столбцов
   {правая линейная комбинация столбцов}%
   {right linear combination of columns}%
\Index%956%П%правая линейная комбинация строк
   {правая линейная комбинация строк}%
   {right linear combination of rows}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%704%П%правый смежный класс
   {правый смежный класс}%
   {right coset}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%974%П%преобразование подобия
   {преобразование подобия}%
   {similarity transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%133%П%произведение гомоморфизмов
   {произведение гомоморфизмов}%
   {product of homomorphisms}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%220%С%система левых AD* линейных уравнений
   {система левых $A_*$\Hyph линейных уравнений}%
   {system of left AD* linear equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%721%С%система правых AU* линейных уравнений
   {система правых $A^*$\Hyph линейных уравнений}%
   {system of right AU* linear equations}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%965%С%собственная строка
   {собственная строка}%
   {eigenrow}%
\Index%946%С%собственное значение
   {собственное значение}%
   {eigenvalue}%
\Index%966%С%собственный вектор
   {собственный вектор}%
   {eigenvector}%
\Index%947%С%собственный столбец
   {собственный столбец}%
   {eigencolumn}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%135%Т%тип геометрического объекта
   {тип геометрического объекта}%
   {type of geometric object}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%724%Т%точная последовательность
   {точная последовательность}%
   {exact sequence}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\Index%972%Т%тривиальное ядро гомоморфизма
   {тривиальное ядро гомоморфизма}%
   {trivial kernel}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%975%У%унитальная алгебра
   {унитальная алгебра}%
   {unital algebra}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%369%Ф%факторгруппа
   {факторгруппа}%
   {factor group}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%722%Ц%центр A числа
   {центр $A$\Hyph числа}%
   {center of A number}%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%971%Я%ядро гомоморфизма групп
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Preface.Monomial.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

%\chapter{Preface}
%\newpage

\section{Linear Map}

\begin{convention}
If the map
%\ShowEq{f:A->B}fHH
%of quaternion algebra $H$
\ShowEq{f:A->B}fAA
of $D$\Hyph algebra $A$
is linear map,
then I use notation
\DrawEq{f circ a =}{21 01 06}
for image of the map $f$.
\qed
\end{convention}

\ShowDefinition{linear map of algebra}

Let $H$ be quaternion algebra.

\ShowTheorem{representation of algebra H2 in LH}
\ShowProof{representation of algebra H2 in LH}

\ShowDefinition{component of linear map, basis E}

\FrameEqRef{linear map f, basis E}1

\ShowDefinition{polylinear map of algebras, property}

%\ShowTheorem{representation of algebra An in LAnA}

\begin{\TheoremStyle}
\labelTheorem{representation of algebra An in LAnA}
A representation
\ShowEq{representation An in LAnA}RH
of algebra \AOn[H]
in module \LAnAB RHH
defined by the equality
\DrawEq[RH]{representation An in LAnA, 1}{RH}
allows us to identify tensor
\ShowEq{product in algebra An 1}
and transposition $\sigma\in S^n$
with map
\DrawEq[RH]{product in algebra An 2}{RH}
where
\ShowEq{product in algebra AA 3}RH{\delta}
is identity map.
\end{\TheoremStyle}

\section{Polynomial}

\begin{\DefinitionStyle}
Let
\ShowEq{f:A->B}f{A^n}A
be polylinear map of $D$\Hyph module $A$.
The map
\ShowEq{f:A->B}pAA
defined by the equality
\ShowEq{pxn=fx1...n}
is called
\AddIndex{homogeneous polynomial}{homogeneous polynomial}
of power $n$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
The set
\ShowEq{set of homogeneous polynomials}n
of homogeneous polynomials of power $n$
is Abelian group.
\end{\TheoremStyle}

\begin{proof}
The theorem follows from the statement
that sum of $n$\Hyph linear maps
is $n$\Hyph linear map.
\end{proof}

\begin{\TheoremStyle}
Let $A$ be $D$\Hyph algebra.
Then for any homogeneous polynomial
\ShowEq{f:A->B}pAA
of power $n$
there exists tensor
\ShowEq{p' in An+1}
such that
\ShowEq{pox=p'ox}
\end{\TheoremStyle}

\begin{proof}
The theorem follows the theorem
\RefTheorem{representation of algebra An in LAnA}.
Hereinafter we will identify homogeneous polynomial $p$
and corresponding tensor $p'$.
\end{proof}

\begin{\DefinitionStyle}
If the tensor $p$ has form
\ShowEq{p=p1 ox...ox pn}
then polynomial $p\circ x^n$ is called monomial.
\end{\DefinitionStyle}

\ProveTheorem{monomial of power k}

\ShowRemark{monomial of power k}

\begin{\DefinitionStyle}
\labelDefinition{Polynomial over algebra}
We denote
\ShowEq{algebra of polynomials over algebra}
direct sum\,\footnotemark
of Abelian groups $A_n[x]$.
An element $p(x)$ of Abelian group $A[x]$ is called
\AddIndex{polynomial}{polynomial}
over $D$\Hyph algebra $A$.
\end{\DefinitionStyle}
\footnotetext{\,
See the definition
of direct sum of Abelian groups in
\citeBib{Serge Lang}, pages 36, 37.
On the same page, Lang proves the existence of direct sum of Abelian groups.
}

Therefore, we can present polynomial of power $n$ in the following form
\DrawEq[pn]{p(x)=sum p circ xk}1

\section{Operations with Polynomials}

\begin{\DefinitionStyle}
Let
\DrawEq[pn]{p(x)=sum p circ xk}{}
\DrawEq[rn]{p(x)=sum p circ xk}{}
be polynomials.\,\footnotemark
We introduce the sum of polynomials $p$ and $r$ by the equality
\ShowEq{p+r(x)=sum}
\end{\DefinitionStyle}
\footnotetext{\,
If the coefficient, let's say $p_i$,
is absent, then we assume $p_i=0$.
}

\ShowDefinition{polynomial*polynomial}

\ShowTheorem{(a*b)x=(ax)(bx)}

\section{Linear Equation}

Let $\Basis e$ be the basis of finite dumentional algebra $A$ over field $F$ and
\ShowEq{structural constants of algebra}
be structural constants of algebra $A$
relative to the basis $\Basis e$.

Consider the linear equation
\DrawEq{a circ x=b}0
where
\ShowEq{a in A2}
According to the theorem
\RefTheorem[\RefLinearMap]{standard representation of map A1 A2, associative algebra},
we can write the equation
\eqRef{a circ x=b}0
in standard form
\DrawEq{linear equation in associative algebra, standard form}1
\ShowEq{linear equation in associative algebra, standard form, aij=}
According to the theorem
\RefTheorem[\RefLinearMap]{coordinates of map A1 A2, algebra},
equation
\eqRef{linear equation in associative algebra, standard form}1
is equivalent to equation
\ShowEq{linear equation in associative algebra over field}
\ShowEq{linear equation in associative algebra over field, aij=}
According to
the theory of linear equations over field,
if determinant
\ShowEq{determinant of linear equation in associative algebra over field}
then equation
\eqRef{a circ x=b}0
has only one solution.

\FrameEqRef{a circ x=b}0

\FrameCiteBib{1502.04063}

\begin{\DefinitionStyle}
\labelDefinition{nonsingular tensor}
The tensor
\ShowEq{a in A2ox}
is called
\AddIndex{nonsingular tensor}{nonsingular tensor}
if this tensor satisfies to condition
\EqRef{determinant of linear equation in associative algebra over field}.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{nonsingular tensor}
Let
\ShowEq{a in A2ox}
be nonsingular tensor.
If we consider the equation
\eqRef{linear equation in associative algebra, standard form}1
as transformation of algebra $A$, then we can write the inverse transformation
in form
\ShowEq{linear equation in associative algebra, root, 1}
where components $c^{\gi{pq}}$ satisfy to equation
\ShowEq{linear equation in associative algebra, root}
\end{\TheoremStyle}
\ProofTheorem{1302.7204}{nonsingular tensor}

\FrameEqRef{a circ x=b}0
\FrameEqRef{linear equation in associative algebra, standard form}1

\FrameCiteBib{1302.7204}

\begin{\DefinitionStyle}
\labelDefinition{inverse tensor}
Let
\ShowEq{a in A2ox}
be nonsingular tensor.
The tensor
\ShowEq{inverse tensor}
\ShowEq{def inverse tensor}
is called
\AddIndex{tensor inverse to tensor}{inverse tensor}
$a$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
Let
\ShowEq{a in A2ox}
be nonsingular tensor.
Then linear equation
\DrawEq{a circ x=b}1
has unique solution
\ShowEq{x=a- o b}
If $a$ is singular tensor,
then the equation
\eqRef{a circ x=b}1
has solution only when
\ShowEq{b in ker a}
In this case the equation
\eqRef{a circ x=b}1
has infinitely many solutions.
\end{\TheoremStyle}

\FrameEqRef{a circ x=b}1

\begin{\ExampleStyle}
The tensor
\ShowEq{1 ox i-i ox 1}
corresponds to the matrix
\ShowEq{1 ox i-i ox 1 matrix}
Therefore,
\ShowRemark{ix-xi-1 roots}1k
\end{\ExampleStyle}

\section{Left-sided Polynomial}

\FrameCiteBib{Cohn: Skew Fields}

In the book
\citeBib{Cohn: Skew Fields}
on the page 48,
professor Cohn wrote that the study
of polynomials over skew field is difficult problem.
For this reason professor Ore considered
skew right polynomial ring\,\footnote{\,
See also the definition on pages
\citeBib{Cohn: Skew Fields}\Hyph(48 - 49).
}
where Ore introduced the transformation of monomial
\ShowEq{at=taa+ad}
The map
\ShowEq{map a in A}{\alpha}
is endomorphism of $D$\Hyph algebra $A$
and the map
\ShowEq{map a in A}{\delta}
is $\alpha$\Hyph derivation of $D$\Hyph algebra $A$
\ShowEq{alpha derivation of algebra}
In such case
all coefficients of polynomial can be written on the right.
Such polynomials are called right\Hyph sided polynomials.

The same way we may consider
the transformation of monomial
\ShowEq{ta=aat+ad}
In such case
all coefficients of polynomial can be written on the left.
Such polynomials are called left\Hyph sided polynomials.\,\footnote{\,
See also the definition on the page
\citeBib{1702.04935}\Hyph 3.
}

The point of view proposed by Ore
allows us to get qualitative picture of the theory
of polynomials in non\Hyph commutative algebra.
However, there exist algebras where this point of view is not complete.

\begin{\ExampleStyle}
If there exist transformation
\EqRef{at=taa+ad}
in $D$\Hyph algebra $A$,
then we can map any polynomial $p$ of power $1$
into right\Hyph sided polynomial $p'$ of power $1$
such way that
\[p(t)=p'(t)\]
The polynomial $p'$ may have the following form
\ShowEq{p' ta+b}
\ShowEq{p' t0+b}
\ShowEq{p' t0+0}
The polynomial
\EqRef{p' ta+b}
has unique solution.
The polynomial
\EqRef{p' t0+b}
has no solution.
Any $A$\Hyph number is root of the polynomial
\EqRef{p' t0+0}.

It is evident that we missed the case
when the polynomial $p$ has infinitely many roots,
but not any $A$\Hyph number is the root of the polynomial $p$.
Therefore the question about the existence of transformation
\EqRef{at=taa+ad}
in quaternion algebra
arises.
\end{\ExampleStyle}

\ShowExample{polynomial p*r(x)}


==> Preface.Monomial.Eq.tex <==
%auto-ignore
\Input{Stmt.2021.11.26}

\AddEq{a in A2}
{
$a=a_{s\cdot 0}\otimes a_{s\cdot 1}\in A^{2\otimes}$.
}

\AddEq{linear equation in associative algebra, standard form}
{
\aU a{ij}\aD eix\aD ej=b
}

\AddEquation{linear equation in associative algebra, standard form, aij=}
{
\begin{matrix}
\aU a{ij}=a_{s\cdot}{}{}_0^{\gi i}\,a_{s\cdot}{}{}_1^{\gi j}
&a_{s\cdot 0}=a_{s\cdot}{}{}_0^{\gi i}e_{\gi i}
&a_{s\cdot 1}=a_{s\cdot}{}{}_1^{\gi i}e_{\gi i}
\end{matrix}
}

\AddEquation{linear equation in associative algebra over field}
{
\aUD aji\aU xi=\aU bj
}

\AddEquation{linear equation in associative algebra over field, aij=}
{
\begin{matrix}
\aUD aji=\aU a{kr}\aUD Cp{ki}\aUD Cj{pr}
&x=\aU xi\aD ei
&b=\aU bi\aD ei
\end{matrix}
}

\AddEquation{linear equation in associative algebra, root, 1}
{
x=\aU c{pq}\aD epb\aD eq
}

\AddEquation{linear equation in associative algebra, root}
{
\aUD{\delta}r0\aUD{\delta}s0
=\aU a{ij}\aU c{pq}\aUD Cr{ip}\aUD Cs{qj}
}

\AddEquation{at=taa+ad}
{
at=ta^{\alpha}+a^{\delta}
}

\AddEquation{ta=aat+ad}
{
ta=a^{\alpha}t+a^{\delta}
}

\AddEquation{p' ta+b}
{
p'(t)=ta_1+a_0\ \ \ \ a_1\ne 0
}

\AddEquation{p' t0+b}
{
p'(t)=t\,0+a_0\ \ \ \ a_0\ne 0
}

\AddEquation{p' t0+0}
{
p'(t)=t\,0+0
}

\AddEquation{alpha derivation of algebra}
{
(a+b)^{\delta}=a^{\delta}+b^{\delta}
\ \ \ \ (ab)^{\delta}=a^{\delta}b^{\alpha}+ab^{\delta}
}

\AddEq[1]{map a in A}
{
\ShowEq{f:a in A->b in B}{#1}aA{a^{#1}}A
}

\AddEquation{x=a- o b}
{
x=a^{-1}\circ b
}

\AddEq{b in ker a}
{
$b\in\ker a$.
}

\AddEq{inverse tensor}
{
\symb{a^{-1}}{inverse tensor}{}
}

\AddEquation{def inverse tensor}
{
\ShowSymbol{inverse tensor}{}=
c^{\gi{pq}}e_{\gi p}\otimes e_{\gi q}
}

\AddEquation{determinant of linear equation in associative algebra over field}
{
\det\|\aUD aji\|\ne 0
}

\AddEq{a in A2ox}
{
$a\in A^{2\otimes}$
}

\AddEq{p=p1 ox...ox pn}
{
$p=p_0\otimes...\otimes p_n$,
}

\AddEquation{p+r(x)=sum}
{
(p+r)(x)=p_0+r_0+(p_1+r_1)\circ x+...+(p_n+r_n)\circ x^n
}

\AddEq[2]{p(x)=sum p circ xk}
{
\begin{matrix}
#1(x)=#1_0+#1_1\circ x+...+#1_{#2}\circ x^{#2}
&#1_i\in A^{i+1\otimes}&i=0,...,n
\end{matrix}
}

\AddEq{p' in An+1}
{
$p'\in\AOn$
}

\AddEquation{pox=p'ox}
{
p\circ x^n=p'\circ x^n=p'\circ(x_1,...,x_n)
\ \ \ \ x_1=...=x_n=x
}

\AddEquation{pxn=fx1...n}
{
p\circ x^n=f\circ(x_1,...,x_n)\ \ \ \ x_1=...=x_n=x
}


==> Preface.Monomial.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

%\chapter{Предисловие}
%\newpage

\section{Линейное отображение}

\begin{convention}
Если отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
является линейным отображением,
то я пользуюсь обозначением
\DrawEq{f circ a =}{21 01 06}
для образа отображения $f$.
\qed
\end{convention}

\ShowDefinition{linear map of algebra}

Пусть $H$ - алгебра кватернионов.

\ShowTheorem{representation of algebra H2 in LH}
\ShowProof{representation of algebra H2 in LH}

\ShowDefinition{component of linear map, basis E}

\FrameEqRef{linear map f, basis E}1

\ShowDefinition{polylinear map of algebras, property}

%\ShowTheorem{representation of algebra An in LAnA}

\begin{\TheoremStyle}
\labelTheorem{representation of algebra An in LAnA}
Представление
\ShowEq{representation An in LAnA}RH
алгебры \AOn[H]
в модуле \LAnAB RHH,
определённое равенством
\DrawEq[RH]{representation An in LAnA, 1}{RH}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[RH]{product in algebra An 2}{RH}
где
\ShowEq{product in algebra AA 3}RH{\delta}
- тождественное отображение.
\end{\TheoremStyle}

\section{Многочлен}

\begin{\DefinitionStyle}
Пусть
\ShowEq{f:A->B}f{A^n}A
полилинейное отображение $D$\Hyph модуля $A$.е
Отображение
\ShowEq{f:A->B}pAA
определённое равенством
\ShowEq{pxn=fx1...n}
называется
\AddIndex{однородным многочленом}{homogeneous polynomial}
степени $n$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
Множество
\ShowEq{set of homogeneous polynomials}n
однородных многочленов степени $n$
является абелевой группой.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием утверждения,
что сумма $n$\Hyph линейных отображений
является $n$\Hyph линейным отображением.
\end{proof}

\begin{\TheoremStyle}
Пусть $A$ - $D$\Hyph алгебра.
Тогда для любого однородного многочлена
\ShowEq{f:A->B}pAA
степени $n$
существует тензор
\ShowEq{p' in An+1}
такой, что
\ShowEq{pox=p'ox}
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием теоремы
\RefTheorem{representation of algebra An in LAnA}.
В дальнейшем мы будем отождествлять однородный многочлен $p$
и соответствующий тензор $p'$.
\end{proof}

\begin{\DefinitionStyle}
Если тензор $p$ имеет вид
\ShowEq{p=p1 ox...ox pn}
то многочлен $p\circ x^n$ называется одночленом.
\end{\DefinitionStyle}

\ProveTheorem{monomial of power k}

\ShowRemark{monomial of power k}

\begin{\DefinitionStyle}
\labelDefinition{Polynomial over algebra}
Обозначим
\ShowEq{algebra of polynomials over algebra}
прямую сумму\,\footnotemark
абелевых групп $A_n[x]$.
Элемент $p(x)$ абелевой группы $A[x]$ называется
\AddIndex{многочленом}{polynomial}
над $D$\Hyph алгеброй $A$.
\end{\DefinitionStyle}
\footnotetext{\,
Смотри определение
прямой суммы абелевых групп в
\citeBib{Serge Lang}, страница 55.
Согласно теореме 1 на той же странице, прямая сумма абелевых групп существует.
}

Следовательно, многочлен степени $n$ может быть записан в виде
\DrawEq[pn]{p(x)=sum p circ xk}1

\section{Операции с многочленами}

\begin{\DefinitionStyle}
Пусть
\DrawEq[pn]{p(x)=sum p circ xk}{}
\DrawEq[rn]{p(x)=sum p circ xk}{}
многочлены.\,\footnotemark
Мы определим сумму многочленов $p$ и $r$ равенством
\ShowEq{p+r(x)=sum}
\end{\DefinitionStyle}
\footnotetext{\,
Если коэффициент, допустим $p_i$,
отсутствует, то мы полагаем $p_i=0$.
}

\ShowDefinition{polynomial*polynomial}

\ShowTheorem{(a*b)x=(ax)(bx)}

\section{Линейное уравнение}

Пусть $\Basis e$ - базис конечно мерной алгебры $A$ над полем $F$ и
\ShowEq{structural constants of algebra}
- структурные константы алгебры $A$
относительно базиса $\Basis e$.

Рассмотрим линейное уравнение
\DrawEq{a circ x=b}0
где
\ShowEq{a in A2}
Согласно теореме
\RefTheorem[\RefLinearMap]{standard representation of map A1 A2, associative algebra},
мы можем записать уравнение
\eqRef{a circ x=b}0
в стандартной форме
\DrawEq{linear equation in associative algebra, standard form}1
\ShowEq{linear equation in associative algebra, standard form, aij=}
Согласно теореме
\RefTheorem[\RefLinearMap]{coordinates of map A1 A2, algebra},
уравнение
\eqRef{linear equation in associative algebra, standard form}1
эквивалентно уравнению
\ShowEq{linear equation in associative algebra over field}
\ShowEq{linear equation in associative algebra over field, aij=}
Согласно
теории линейных уравнений над полем,
если определитель
\ShowEq{determinant of linear equation in associative algebra over field}
то уравнение
\eqRef{a circ x=b}0
имеет единственное решение.

\FrameEqRef{a circ x=b}0

\FrameCiteBib{1502.04063}

\begin{\DefinitionStyle}
\labelDefinition{nonsingular tensor}
Тензор
\ShowEq{a in A2ox}
называется
\AddIndex{невырожденным тензором}{nonsingular tensor},
если этот тензор удовлетворяет условию
\EqRef{determinant of linear equation in associative algebra over field}.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{nonsingular tensor}
Пусть
\ShowEq{a in A2ox}
- невырожденный тензор.
Если равенство
\eqRef{linear equation in associative algebra, standard form}1
рассматривать как преобразование алгебры $A$, то обратное преобразование
можно записать в виде
\ShowEq{linear equation in associative algebra, root, 1}
где компоненты $c^{\gi{pq}}$ удовлетворяют уравнению
\ShowEq{linear equation in associative algebra, root}
\end{\TheoremStyle}
\ProofTheorem{1302.7204}{nonsingular tensor}

\FrameEqRef{a circ x=b}0
\FrameEqRef{linear equation in associative algebra, standard form}1

\FrameCiteBib{1302.7204}

\begin{\DefinitionStyle}
\labelDefinition{inverse tensor}
Пусть
\ShowEq{a in A2ox}
- невырожденный тензор.
Тензор
\ShowEq{inverse tensor}
\ShowEq{def inverse tensor}
называется
\AddIndex{тензором, обратным тензору}{inverse tensor}
$a$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
Если
\ShowEq{a in A2ox}
- невырожденный тензор,
то линейное уравнение
\DrawEq{a circ x=b}1
имеет единственное решение
\ShowEq{x=a- o b}
Если $a$- невырожденный тензор,
то уравнение
\eqRef{a circ x=b}1
имеет решение только при условии
\ShowEq{b in ker a}
В этом случае уравнение
\eqRef{a circ x=b}1
имеет бесконечно много решений.
\end{\TheoremStyle}

\FrameEqRef{a circ x=b}1

\begin{\ExampleStyle}
Тензор
\ShowEq{1 ox i-i ox 1}
соответствует матрице
\ShowEq{1 ox i-i ox 1 matrix}
Следовательно
\ShowRemark{ix-xi-1 roots}1k
\end{\ExampleStyle}

\section{Левостороний многочлен}

\FrameCiteBib{Cohn: Skew Fields}

В книге
\citeBib{Cohn: Skew Fields}
на странице 48,
профессор Кон писал, что изучать многочлены
над не коммутативным полем - сложная задача.
Поэтому профессор Оре рассмотрел
кольцо правых косых многочленов\,\footnote{\,
Смотри также определение на страницах
\citeBib{Cohn: Skew Fields}\Hyph(48 - 49).
}
где Оре определил преобразование одночлена
\ShowEq{at=taa+ad}
Отображение
\ShowEq{map a in A}{\alpha}
является эндоморфизмом $D$\Hyph алгебры $A$
и отображение
\ShowEq{map a in A}{\delta}
является $\alpha$\Hyph дифференцированием $D$\Hyph алгебры $A$
\ShowEq{alpha derivation of algebra}
В этом случае
все коэффициенты многочлена могут быть записаны справа.
Подобные многочлены называются правостороними многочленами.

Аналогично мы можем рассматривать
преобразование одночлена
\ShowEq{ta=aat+ad}
В этом случае
все коэффициенты многочлена могут быть записаны слева.
Подобные многочлены называются левостороними многочленами.\,\footnote{\,
Смотри также определение на странице
\citeBib{1702.04935}\Hyph 3.
}

Точка зрения, предложенная Оре,
позволила получить качественную картину теории
полиномов в некоммутативной алгебре.
Однако существуют алгебры где рассматриваемая картина не полна.

\begin{\ExampleStyle}
Если преобразование
\EqRef{at=taa+ad}
определено в $D$\Hyph алгебре $A$,
то мы можем любой многочлен $p$ степени $1$
отобразить в правостороний многочлен $p'$ степени $1$
таким образом, что
\[p(t)=p'(t)\]
Многочлен $p'$ может иметь следующий вид
\ShowEq{p' ta+b}
\ShowEq{p' t0+b}
\ShowEq{p' t0+0}
Многочлен
\EqRef{p' ta+b}
имеет единственное решение.
Многочлен
\EqRef{p' t0+b}
не имеет решений.
Любое $A$\Hyph число является корнем многочлена
\EqRef{p' t0+0}.

Очевидно, что мы упустили случай,
когда многочлен $p$ имеет бесконечно много корней,
но не любое $A$\Hyph число является корнем многочлена $p$.
Поэтому возникает
вопрос о существовании преобразования
\EqRef{at=taa+ad}
в алгебре кватернионов.
\end{\ExampleStyle}

\ShowExample{polynomial p*r(x)}


==> Prolog.Cite.Russian.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}


==> Stmt.2021.11.26.English.tex <==
%auto-ignore
\input{Stmt.2021.11.26.Eq}

\DefExample{r=x2-jx-xi-k p=x-i}
{
Let
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-jx-xi-k}1
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x ox 1}
Then
\ShowEq{s1=r-.p. 1}
Now we set
\ShowEq{q0= 1}
Then
\ShowEq{s0=s-.p. 1}
The equality
\ShowEq{r=x2-jx-xi-k 1}
follows from equalities
\EqRef{s1=r-.p. 1},
\EqRef{s0=s-.p. 1}.
We can reduce expression in the equality
\EqRef{r=x2-jx-xi-k 1}
\ShowEq{r=x2-jx-xi-k 2}
We see that the representation of the polynomial $r(x)$ in the equality
\EqRef{r=x2-jx-xi-k 2}
is the same as the representation of the polynomial $r(x)$ in the equality
\eqRef{r=x2-jx-xi-k}1.
}

\AddEq{remark: r=x2-jx-xi-k p=x-i}
{
The answer
\EqRef{r=x2-jx-xi-k 2}
in the example
\RefExample{r=x2-jx-xi-k p=x-i}
is evident because I intentionally chose divisor $p(x)$
to be equal second factor of the polynomial $r(x)$.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-jx-xi-k}
}

\AddEq{remark: r=x2-ix-xj+k p=x-i}
{
The example
\RefExample{r=x2-ix-xj+k p=x-i}
is more interesting because I considered different order of factors.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-xj+k p=x-i}
Let
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-ix-xj+k}1
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x ox 1}
Then
\ShowEq{s1=r-.p. 2}
Now we set
\ShowEq{q0= 2}
Then
\ShowEq{s0=s-.p. 2}
The equality
\ShowEq{r=x2-ix-xj+k 1}
follows from equalities
\EqRef{s1=r-.p. 2},
\EqRef{s0=s-.p. 2}.
We can reduce expression in the equality
\EqRef{r=x2-ix-xj+k 1}
\ShowEq{r=x2-ix-xj+k 2}
We see that the representation of the polynomial $r(x)$ in the equality
\EqRef{r=x2-ix-xj+k 2}
is the same as the representation of the polynomial $r(x)$ in the equality
\eqRef{r=x2-ix-xj+k}1.
\end{\ExampleStyle}

The quotient of polynomial $r(x)$ divided by polynomial $p(x)$
in the example
\RefExample{r=x2-ix-xj+k p=x-i}
has a more complicated structure than the quotient
in the example
\RefExample{r=x2-jx-xi-k p=x-i}.
This is because I am trying to write down the divisor $p(x)$
to the right of the quotient, although initially the polynomial $p(x)$
was left factor.
Nevertheless, as a result of simple transformations,
factorization in the equality
\EqRef{r=x2-ix-xj+k 2}
took the expected form.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-ix-xj+k}
}

\DefExampleNote{polynomial p*r(x)}
{
Let
\ShowEq{polynomial p(x)}pin
and
\ShowEq{polynomial p(x)}rjm
be left\Hyph sided polynomials.
We introduce product of polynomials $p$ and $r$ by the equality\,\footnotemark
\ShowEq{polynomial p*r(x)}

Consider polynomials
\DrawEq[Li]{Px=x-i}i
\DrawEq[Rj]{Px=x-i}j
The equality
\ShowEq{Px=x-i*x-j}
follows from equalities
\EqRef{polynomial p*r(x)},
\eqRef{Px=x-i}i,
\eqRef{Px=x-i}j.
Let
\ShowEq{h=Ri}
\ShowEq{x-=}
\ShowEq{L(x-)=}
According to the theorem
\citeBib{1702.04935}\Hyph 1, item $(ii)$,
the polynomial
\ShowEq{P1=L(x-)R(x)}
coincides with the polynomial $P(x)$,
$P_1(x)=P(x)$
\ShowEq{p(x)=L(x-)R(x)}

However, the equality
\EqRef{p(x)=L(x-)R(x)}
is not true.
Let $x=i+j$.
Equalities
\ShowEq{p(i+j)=L(i+j-)R(i+j)}
\ShowEq{p(i+j)=L(i+j-)R(i+j) 1}
follow from the equality
\EqRef{p(x)=L(x-)R(x)}.
}
{
See also the definition on the page
\citeBib{1702.04935}\Hyph 3.
}

\AddEq{remark: r=x2-ix-jx-k}
{
In the example
\RefExample{r=x2-ix-jx-k},
I consider division of the left\Hyph sided polynomial
\DrawEq{r=x2-ix-jx-k}{}
over the polynomial
\ShowEq{p=x-i}i
I know that the polynomial $r(x)$ has solution $x=i$
and want to find another solution.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-jx-k}
%.3.
Let
\ShowEq{p=x-i}i
\DrawEq{r=x2-ix-jx-k}{}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x ox 1}
Then
\ShowEq{s1=r-.p. 3}
Now we set
\ShowEq{q0= 3}
Then
\ShowEq{s0=s-.p. 3}
The equality
\ShowEq{r=x2-ix-jx-k 1}
follows from equalities
\EqRef{s1=r-.p. 3},
\EqRef{s0=s-.p. 3}.
We can reduce expression in the equality
\EqRef{r=x2-ix-jx-k 1}
\ShowEq{r=x2-ix-jx-k 10}
\end{\ExampleStyle}
}

\DefQuestion{r=x2-ix-jx-k}
{
Does the polynomial
\DrawEq{r=x2-ix-jx-k}{}
have root different from $x=i$?
}

\AddEq{remark: r=x2-ix-jx-k 1}
{
We verify immediately that
$x=i$ is the root of the polynomial $r(x)$.
According to the example
\RefExample{r=x2-ix-jx-k},
we can represent the polynomial $r(x)$ as
\DrawEq{r=x2-ix-jx-k 2}2
Therefore, in order for the polynomial $p(x)$ to have
the root different from $x=i$,
it is necessary that linear map
\DrawEq{r=x2-ix-jx-k map}1
has non\Hyph trivial kernel
and quaternion $x-i$
belongs to the kernel of the linear map
\eqRef{r=x2-ix-jx-k map}1.
The linear map
\eqRef{r=x2-ix-jx-k map}1
has the matrix
\ShowEq{r=x2-ix-jx-k matrix}
Search of a value of $x$ for which the matrix
\EqRef{r=x2-ix-jx-k matrix}
is not singular is not simple task.
However I hope to do research in this direction.
}

\AddEq{remark: r=x2-ix-jx-k p=x-j}
{
In the example
\RefExample{r=x2-ix-jx-k p=x-j},
I consider division of the left\Hyph sided polynomial
\ShowEq{r=x2-ix-jx-k  r(j)=}
over the polynomial
\ShowEq{p=x-i}j
}

\DefExample{r=x2-ix-jx-k p=x-j}
{
%.3j.
Let
\ShowEq{p=x-i}j
\DrawEq{r=x2-ix-jx-k}{}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x ox 1}
Then
\ShowEq{s1=r-.p. 3j}
Now we set
\ShowEq{q0= 3j}
Then
\ShowEq{s0=s-.p. 3j}
The equality
\ShowEq{r=x2-ix-jx-k 3j}
follows from equalities
\EqRef{s1=r-.p. 3j},
\EqRef{s0=s-.p. 3j}.
We can reduce expression in the equality
\EqRef{r=x2-ix-jx-k 3j}
\ShowEq{r=x2-ix-jx-k 3j 1}
}

\AddEq{remark: r=(x-j)(x-k)(x-j-k)}
{
In the example
\RefExample{r=(x-j)(x-k)(x-j-k)},
I considered the polynomial $r(x)$ of power $3$
in order to find quotient of the polynomial $r(x)$ divided by two polynomials.
First I will find a quotient of the polynomial
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
divided by the polynomial
\ShowEq{p=x-i}k

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-j-k)}
Let
\ShowEq{p=x-i}k
\ShowEq{r=(x-j)(x-k)(x-j-k)}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q2=x2 ox 1}
Then
\ShowEq{s2=r-.p. 5}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=... 5}
The equality
\ShowEq{s1=s2-.p. 5}
follows from equalities
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5}.
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q0=... 5}
The equality
\ShowEq{s0=s1-.p. 5}
follows from equalities
\EqRef{s1=s2-.p. 5},
\EqRef{q0=... 5}.
The equality
\ShowEq{r=s0+q1+q2 5}
follows from equalities
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5},
\EqRef{q0=... 5},
\EqRef{s0=s1-.p. 5}.
\end{\ExampleStyle}

The quotient
\ShowEq{q=q1+q2 5}
of the polynomial
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
divided by the polynomial
\ShowEq{p=x-i}k
is a tensor depending on $x$,
not a polynomial.
That is why we cannot use the theorem
\RefTheorem{r=+q circ (x-a)}.
}

\DefQuestion{how to select factor in the tensor}
{
It is easy to see that
\ShowEq{q1+q2 5 x=j}
Therefore, the question arises of how to select in the tensor
\DrawEq{q1+q2 5 x}1
factor $x-j$.
}

\DefExample{select factor in the tensor}
{
One possible answer to the question
\RefQuestion{how to select factor in the tensor}
is the transformation
\ShowEq{q1+q2 5 x,1}
Consider the polinomial
\DrawEq{q1+q2 5 x,3}1
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x ox 1}
Then
\ShowEq{s1=r-.p. 7}
Now we set
\ShowEq{q0= 7}
Then
\ShowEq{s0=s-.p. 7}
The equality
\ShowEq{r=x2... 7}
follows from equalities
\EqRef{s1=r-.p. 7},
\EqRef{s0=s-.p. 7}.
The equality
\ShowEq{q1+q2 5 x,2}
follows from equalities
\EqRef{q1+q2 5 x,1},
\EqRef{r=x2... 7}.
}

\AddEq{remark: select factor in the tensor}
{
We see that quotient in the example
\RefExample{select factor in the tensor}
is $H^{3\otimes}$\Hyph number.
}

\DefExample{factorization as bilinear map}
{
The equality
\ShowEq{r= 8}
follows from equalities
\EqRef{r=s0+q1+q2 5},
\EqRef{q1+q2 5 x,2}.
}

\DefQuestion{factorization as bilinear map}
{
The equality
\EqRef{r= 8}
is an answer to the question
\RefQuestion{how to select factor in the tensor}.
We see that factorization of the polynomial $r(x)$
is bilinear map of polynomial
$x-j$, $x-k$.
However this answer is not complete.
According to the remark
\RefRemark{monomial of power k},
the representation
\EqRef{r=+q circ p}
of polynomial is not unique.
The question of the choice of factors and their order is open.
At the same time there is relation between different representations of polynomial
as product of factors.
}


==> Stmt.2021.11.26.Eq.tex <==
%auto-ignore

\AddEq{p=x-i Red}
{
p(x)=\RedText{x-i}
}

\AddEq[1]{p=x-i}
{
\[
p(x)=x-#1
\]
}

\AddEq{r=x2-jx-xi-k}
{
r(x)=(x-j)(\RedText{x-i})=x^2-jx-xi-k
}

\AddEq{r=x2-ix-xj+k}
{
r(x)=(\RedText{x-i})(x-j)=x^2-ix-xj+k
}

\AddEquation{s1=r-.p. 1}
{
\begin{split}
s_1(x)&=r(x)-q_1(x)\circ p(x)=r(x)-(x\otimes 1)\circ(x-i)\\
&=x^2-jx-xi-k-x(x-i)
=x^2-jx-xi-k-x^2+xi\\
&=-jx-k
\end{split}
}

\AddEq{q0= 1}
{
$q_0=-j\otimes 1$.
}

\AddEquation{s0=s-.p. 1}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)-(-i\otimes 1-1\otimes j+1\otimes i)\circ(x-i)\\
&=-ix-xj+k+xi+i(x-i)+(x-i)j-(x-i)i\\
&=-ix-xj+k+xi+ix+1+xj-k-xi-1=0
\end{split}
}

\AddEquation{r=x2-jx-xi-k 1}
{
\begin{split}
\EqText{r(x)}&=s_1(x)+(x\otimes 1)\circ(x-i)\\
&=\EqText{(-j\otimes 1+x\otimes 1)\circ(x-i)}
\end{split}
}

\AddEquation{r=x2-jx-xi-k 2}
{
\EqText{r(x)}=((x-j)\otimes 1)\circ(x-i)
=(x-j)(x-i)
}

\AddEq{q1=x ox 1}
{
$q_1(x)=x\otimes 1$.
}

\AddEquation{s1=r-.p. 7}
{
\begin{split}
s_1(x)&=r(x)-q_1(x)\circ (x-j)=r(x)-(x\otimes 1)\circ(x-j)\\
&=
\ShowEq{q1+q2 5 x,3}
-x^2+xj\\
&=i-jx-xk+xj
\end{split}
}

\AddEquation{q0= 7}
{
q_0=-j\otimes 1-1\otimes k+1\otimes j
}

\AddEquation{s0=s-.p. 7}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)
-(-j\otimes 1-1\otimes k+1\otimes j)\circ(x-j)\\
=&i-jx-xk+xj
+j(x-j)+(x-j)k-(x-j)j\\
=&i-jx-xk+xj
+jx-j^2+xk-jk-xj+j^2\\
=&i-jk=0
\end{split}
}

\AddEquation{r=x2... 7}
{
\begin{split}
\EqText{r(x)}&=s_1(x)+(x\otimes 1)\circ(x-j)\\
&=\EqText{(-j\otimes 1-1\otimes k+1\otimes j+x\otimes 1)\circ(x-j)}
\end{split}
}

\AddEquation{q1+q2 5 x,2}
{
\begin{split}
&\ShowEq{q1+q2 5 x}\\
=&-(x-j)\otimes j+(
(-j\otimes 1-1\otimes k+1\otimes j+x\otimes 1)\circ(x-j)
)\otimes 1\\
=&(
(-1\otimes j-j\otimes 1-1\otimes k+1\otimes j+x\otimes 1)\circ(x-j)
)\otimes 1\\
=&(
(-j\otimes 1-1\otimes k+x\otimes 1)\circ(x-j)
)\otimes 1
\end{split}
}

\AddEquation{r= 8}
{
\begin{split}
r(x)
&=((
(-j\otimes 1-1\otimes k+1\otimes j+x\otimes 1)\circ(x-j)
)\otimes 1
)\circ(x-k)\\
&=(
-j\otimes 1\otimes 1-1\otimes k\otimes 1+1\otimes j\otimes 1+x\otimes 1\otimes 1
)\circ(x-j,x-k)
\end{split}
}

\AddEquation{s1=r-.p. 3j}
{
\begin{split}
s_1(x)&=r(x)-(x\otimes 1)\circ(x-i)\\
&=x^2-ix-jx-k-x(x-j)
=x^2-ix-jx-k-x^2+xj\\
&=-ix-jx-k+xj
\end{split}
}

\AddEquation{q0= 3j}
{
q_0=-i\otimes 1-j\otimes 1+1\otimes j
}

\AddEquation{s0=s-.p. 3j}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)-(-i\otimes 1-j\otimes 1+1\otimes j)\circ(x-j)\\
&=-ix-jx-k+xj+i(x-j)+j(x-j)-(x-j)j\\
&=-ix-jx-k+xj+ix-k+jx+1-xj-1=-2k
\end{split}
}

\AddEquation{r=x2-ix-jx-k 3j}
{
\begin{split}
\EqText{r(x)}&=s_1(x)+(x\otimes 1)\circ(x-j)\\
&=s_0+q_0\circ(x-j)+(x\otimes 1)\circ(x-j)\\
&=\EqText{-2k+(-i\otimes 1-j\otimes 1+1\otimes j+x\otimes 1)\circ(x-j)}
\end{split}
}

\AddEquation{r=x2-ix-jx-k 3j 1}
{
r(x)=-2k+(1\otimes j+(x-i-j)\otimes 1)\circ(x-j)
}

\AddEquation{q1+q2 5 x=j}
{
\begin{split}
q(j)&=(
\ShowEq{q1+q2 5 x}
)(j)\\
&=j\otimes j+i\otimes 1
-j\otimes j-j^2\otimes 1-jk\otimes 1
+j^2\otimes 1
=0
\end{split}
}

\AddEq{q1+q2 5 x}
{
j\otimes j+i\otimes 1
-x\otimes j-jx\otimes 1-xk\otimes 1
+x^2\otimes 1
}

\AddEquation{q1+q2 5 x,1}
{
\begin{split}
&\ShowEq{q1+q2 5 x}\\
=&
j\otimes j-x\otimes j+i\otimes 1
-jx\otimes 1-xk\otimes 1
+x^2\otimes 1\\
=&-(x-j)\otimes j+(
\ShowEq{q1+q2 5 x,3}
)\otimes 1
\end{split}
}

\AddEq{q1+q2 5 x,3}
{
i-jx-xk+x^2
}

\AddEq{r=(x-j)(x-k)(x-j-k) 0}
{
\[
r(x)=
\ShowEq{(x-j)(x-k)(x-j-k)}
\]
}

\AddEq{(x-j)(x-k)(x-j-k)}
{
(x-j)(x-k)(x-j-k)
}

\AddEq{r=(x-j)(x-k)(x-j-k)}
{
\begin{align*}
r(x)&=
\ShowEq{(x-j)(x-k)(x-j-k)}
=(x^2-jx-xk+i)(x-j-k)\\
&=x^2(x-j-k)
-jx(x-j-k)
-xk(x-j-k)
+i(x-j-k)\\
&=x^3-x^2j-x^2k
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j\\
&=x^3\\
&+(-1\otimes 1\otimes j-1\otimes 1\otimes k-j\otimes 1\otimes 1-1\otimes k\otimes 1)\circ x^2\\
&+(j\otimes j+j\otimes k-1\otimes i-1\otimes 1+i\otimes 1)\circ x\\
&-k+j
\end{align*}
}

\AddEq{q2=x2 ox 1}
{
$q_2(x)=(x^2)\otimes 1$.
}

\AddEquation{s2=r-.p. 5}
{
\begin{split}
s_2(x)&=r(x)-q_2(x)\circ(x-k)=r(x)-(x^2\otimes 1)\circ(x-k)\\
&=x^3-x^2j-x^2k
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j\\ &-x^3+x^2k\\
&=-x^2j
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j
\end{split}
}

\AddEquation{q1=... 5}
{
q_1(x)=-x\otimes j-jx\otimes 1-xk\otimes 1
}

\AddEquation{s1=s2-.p. 5}
{
\begin{split}
s_1(x)&=s_2(x)-q_1(x)\circ(x-k)\\
&=-x^2j
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j\\
&-(-x\otimes j-jx\otimes 1-xk\otimes 1)\circ(x-k)\\
&=-x^2j
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j\\
&+x(x-k)j+jx(x-k)+xk(x-k)\\
&=-x^2j
-jx^2+jxj+jxk
-xkx+xkj-x
+ix-k+j\\
&+x^2j-xkj+jx^2-jxk+xkx-xkk\\
&=jxj+ix-k+j
\end{split}
}

\AddEquation{q0=... 5}
{
q_0(x)=j\otimes j+i\otimes 1
}

\AddEquation{s0=s1-.p. 5}
{
\begin{split}
s_0&=s_1(x)-q_0(x)\circ(x-k)\\
&=jxj+ix-k+j-(j\otimes j+i\otimes 1)\circ(x-k)\\
&=jxj+ix-k+j-j(x-k)j-i(x-k)\\
&=jxj+ix-k+j-jxj+jkj-ix+ik\\
&=-k+j+jkj+ik=0
\end{split}
}

\AddEquation{q=q1+q2 5}
{
q(x)=
\ShowEq{q1+q2 5 x}
}

\AddEquation{r=s0+q1+q2 5}
{
\begin{split}
r(x)&=s_0+(q_0+q_1(x)+q_2(x))\circ(x-k)\\
&=(
\ShowEq{q1+q2 5 x}
)\circ(x-k)
\end{split}
}

\AddEquation{s1=r-.p. 3}
{
\begin{split}
s_1(x)&=r(x)-(x\otimes 1)\circ(x-i)\\
&=x^2-ix-jx-k-x(x-i)
=x^2-ix-jx-k-x^2+xi\\
&=-ix-jx-k+xi
\end{split}
}

\AddEquation{q0= 3}
{
q_0=-i\otimes 1-j\otimes 1+1\otimes i
}

\AddEquation{s0=s-.p. 3}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)-(-i\otimes 1-j\otimes 1+1\otimes i)\circ(x-i)\\
&=-ix-jx-k+xi+i(x-i)+j(x-i)-(x-i)i\\
&=-ix-jx-k+xi+ix+1+jx+k-xi-1=0
\end{split}
}

\AddEquation{r=x2-ix-jx-k 1}
{
\begin{split}
\EqText{r(x)}&=s_1(x)+(x\otimes 1)\circ(x-i)=q_0\circ(x-i)+(x\otimes 1)\circ(x-i)\\
&=\EqText{(-i\otimes 1-j\otimes 1+1\otimes i+x\otimes 1)\circ(x-i)}
\end{split}
}

\AddEq{r=x2-ix-jx-k 2}
{
r(x)=(
\ShowEq{r=x2-ix-jx-k map}
)\circ (x-i)
}

\AddEq{r=x2-ix-jx-k map}
{
1\otimes i+(x-i-j)\otimes 1
}

\AddEquation{r=x2-ix-jx-k matrix}
{
\begin{split}
&
\begin{pmatrix}
0&-1&0&0\\
1&0&0&0\\
0&0&0&1\\
0&0&-1&0
\end{pmatrix}
+
\begin{pmatrix}
\aU x0&-\aU x1+1&-\aU x2+1&-\aU x3\\
\aU x1-1&\aU x0&-\aU x3&\aU x2-1\\
\aU x2-1&\aU x3&\aU x0&-\aU x1+1\\
\aU x3&-\aU x2+1&\aU x1-1&\aU x0
\end{pmatrix}
\\ =&
\begin{pmatrix}
\aU x0&-\aU x1&-\aU x2+1&-\aU x3\\
\aU x1&\aU x0&-\aU x3&\aU x2-1\\
\aU x2-1&\aU x3&\aU x0&-\aU x1+2\\
\aU x3&-\aU x2+1&\aU x1-2&\aU x0
\end{pmatrix}
\end{split}
}

\AddEq{r=x2-ix-jx-k  r(j)=}
{
\[
\ShowEq{r=x2-ix-jx-k}
\ \ \ \ \ \ \ \ r(j)=-2k
\]
}

\AddEquation{s1=r-.p. 2}
{
\begin{split}
s_1(x)&=r(x)-(x\otimes 1)\circ(x-i)\\
&=x^2-ix-xj+k-x(x-i)
=x^2-ix-xj+k-x^2+xi\\
&=-ix-xj+k+xi
\end{split}
}

\AddEquation{q0= 2}
{
q_0=-i\otimes 1-1\otimes j+1\otimes i
}

\AddEquation{s0=s-.p. 2}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)-(-j\otimes 1)\circ(x-i)\\
&=-jx-k+j(x-i)=-jx-k+jx+k=0
\end{split}
}

\AddEquation{r=x2-ix-xj+k 1}
{
\begin{split}
\EqText{r(x)}&=s_1(x)+(x\otimes 1)\circ(x-i)\\
&=\EqText{(-i\otimes 1-1\otimes j+1\otimes i+x\otimes 1)\circ(x-i)}
\end{split}
}

\AddEquation{r=x2-ix-xj+k 2}
{
\begin{split}
r(x)&=-i(x-i)-(x-i)j+(x-i)i+x(x-i)\\
&=(x-i)(i-j)+(x-i)(x-i)\\
&=(x-i)(x-i+i-j)\\
&=(x-i)(x-j)
\end{split}
}

\AddEq{r=x2-ix-jx-k}
{
r(x)=x^2-ix-jx-k
}

\AddEq[2]{Px=x-i}
{
#1(x)=x-#2
}

\AddEquation{Px=x-i*x-j}
{
P(x)=(L*R)(x)=x^2-(i+j)x+k
}

\AddEq{h=Ri}
{
\[h=R(i)=i-j\]
}

\AddEquation{P1=L(x-)R(x)}
{
P_1(x)=L(\tilde{x})R(x)=(\frac 12(i-j)x(j-i)-i)(x-j)
}


==> Stmt.2021.11.26.Russian.tex <==
%auto-ignore
\input{Stmt.2021.11.26.Eq}

\DefExample{r=x2-jx-xi-k p=x-i}
{
Пусть
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-jx-xi-k}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 1}
Теперь мы положим
\ShowEq{q0= 1}
Тогда
\ShowEq{s0=s-.p. 1}
Равенство
\ShowEq{r=x2-jx-xi-k 1}
является следствием равенств
\EqRef{s1=r-.p. 1},
\EqRef{s0=s-.p. 1}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-jx-xi-k 1}
\ShowEq{r=x2-jx-xi-k 2}
Мы видим, что представление многочлена $r(x)$ в равенстве
\EqRef{r=x2-jx-xi-k 2}
совпадает с представление многочлена $r(x)$ в равенстве
\eqRef{r=x2-jx-xi-k}1.
}

\AddEq{remark: r=x2-jx-xi-k p=x-i}
{
Ответ
\EqRef{r=x2-jx-xi-k 2}
в примере
\RefExample{r=x2-jx-xi-k p=x-i}
очевиден, так как я намеренно выбрал делитель $p(x)$
равным второму множителю многочлена $r(x)$.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-jx-xi-k}
}

\AddEq{remark: r=x2-ix-xj+k p=x-i}
{
Пример
\RefExample{r=x2-ix-xj+k p=x-i}
более интересен, так как я изменил порядок множителей.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-xj+k p=x-i}
Пусть
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-ix-xj+k}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 2}
Теперь мы положим
\ShowEq{q0= 2}
Тогда
\ShowEq{s0=s-.p. 2}
Равенство
\ShowEq{r=x2-ix-xj+k 1}
является следствием равенств
\EqRef{s1=r-.p. 2},
\EqRef{s0=s-.p. 2}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-xj+k 1}
\ShowEq{r=x2-ix-xj+k 2}
Мы видим, что представление многочлена $r(x)$ в равенстве
\EqRef{r=x2-ix-xj+k 2}
совпадает с представление многочлена $r(x)$ в равенстве
\eqRef{r=x2-ix-xj+k}1.
\end{\ExampleStyle}

Частное от деления многочлена $r(x)$ на многочлен $p(x)$
в примере
\RefExample{r=x2-ix-xj+k p=x-i}
имеет более сложную структуру чем частное
в примере
\RefExample{r=x2-jx-xi-k p=x-i}.
Это связано с тем, что я пытаюсь записать делитель $p(x)$
справа от частного, хотя изначально многочлен $p(x)$
был левым множителем.
Тем не менее, в результате несложных преобразований
разложение на множители в равенстве
\EqRef{r=x2-ix-xj+k 2}
приняло ожидаемый вид.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-ix-xj+k}
}

\DefExampleNote{polynomial p*r(x)}
{
Пусть
\ShowEq{polynomial p(x)}pin
и
\ShowEq{polynomial p(x)}rjm
левостороние многочлены.
Мы определим произведение многочленов $p$ и $r$ равенством\,\footnotemark
\ShowEq{polynomial p*r(x)}

Рассмотрим многочлены
\DrawEq[Li]{Px=x-i}i
\DrawEq[Rj]{Px=x-i}j
Равенство
\ShowEq{Px=x-i*x-j}
является следствием равенств
\EqRef{polynomial p*r(x)},
\eqRef{Px=x-i}i,
\eqRef{Px=x-i}j.
Пусть
\ShowEq{h=Ri}
\ShowEq{x-=}
\ShowEq{L(x-)=}
Согласно теореме
\citeBib{1702.04935}\Hyph 1, пункт $(ii)$,
многочлен
\ShowEq{P1=L(x-)R(x)}
совпадает с многочленом $P(x)$,
$P_1(x)=P(x)$
\ShowEq{p(x)=L(x-)R(x)}

Однако равенство
\EqRef{p(x)=L(x-)R(x)}
не верно.
Пусть $x=i+j$.
Равенства
\ShowEq{p(i+j)=L(i+j-)R(i+j)}
\ShowEq{p(i+j)=L(i+j-)R(i+j) 1}
являются следствием равенства
\EqRef{p(x)=L(x-)R(x)}.
}
{
Смотри также определение на странице
\citeBib{1702.04935}\Hyph 3.
}

\AddEq{remark: r=x2-ix-jx-k}
{
В примере
\RefExample{r=x2-ix-jx-k}
я рассмотрел деление левосторонего многочлена
\DrawEq{r=x2-ix-jx-k}{}
на многочлен
\ShowEq{p=x-i}i
Я знаю, что многочлен $r(x)$ имеет корень $x=i$,
и хочу найти другой корень.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-jx-k}
%.3.
Пусть
\ShowEq{p=x-i}i
\DrawEq{r=x2-ix-jx-k}{}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 3}
Теперь мы положим
\ShowEq{q0= 3}
Тогда
\ShowEq{s0=s-.p. 3}
Равенство
\ShowEq{r=x2-ix-jx-k 1}
является следствием равенств
\EqRef{s1=r-.p. 3},
\EqRef{s0=s-.p. 3}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-jx-k 1}
\ShowEq{r=x2-ix-jx-k 10}
\end{\ExampleStyle}
}

\DefQuestion{r=x2-ix-jx-k}
{
Имеет ли многочлен
\DrawEq{r=x2-ix-jx-k}{}
корень, отличный от $x=i$?
}

\AddEq{remark: r=x2-ix-jx-k 1}
{
Утверждение, что $x=i$ является корнем многочлена $r(x)$
проверяется непосредственно.
Согласно примеру
\RefExample{r=x2-ix-jx-k},
мы можем представить многочлен $r(x)$ в виде
\DrawEq{r=x2-ix-jx-k 2}2
Следовательно, для того чтобы многочлен $p(x)$
имел корень, отличный от $x=i$,
необходимо чтобы линейное отображение
\DrawEq{r=x2-ix-jx-k map}1
имело нетривиальное ядро
и кватернион $x-i$
принадлежал ядру линейного отображения
\eqRef{r=x2-ix-jx-k map}1.
Линейное отображение
\eqRef{r=x2-ix-jx-k map}1
имеет матрицу
\ShowEq{r=x2-ix-jx-k matrix}
Определить значение $x$, для которого матрица
\EqRef{r=x2-ix-jx-k matrix}
вырождена - задача непростая.
Но я надеюсь провести дополнительное исследование.
}

\AddEq{remark: r=x2-ix-jx-k p=x-j}
{
В примере
\RefExample{r=x2-ix-jx-k p=x-j}
я рассмотрел деление левосторонего многочлена
\ShowEq{r=x2-ix-jx-k  r(j)=}
на многочлен
\ShowEq{p=x-i}j
}

\DefExample{r=x2-ix-jx-k p=x-j}
{
%.3j.
Пусть
\ShowEq{p=x-i}j
\DrawEq{r=x2-ix-jx-k}{}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 3j}
Теперь мы положим
\ShowEq{q0= 3j}
Тогда
\ShowEq{s0=s-.p. 3j}
Равенство
\ShowEq{r=x2-ix-jx-k 3j}
является следствием равенств
\EqRef{s1=r-.p. 3j},
\EqRef{s0=s-.p. 3j}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-jx-k 3j}
\ShowEq{r=x2-ix-jx-k 3j 1}
}

\AddEq{remark: r=(x-j)(x-k)(x-j-k)}
{
В примере
\RefExample{r=(x-j)(x-k)(x-j-k)}
я рассмотрел многочлен $r(x)$ степени $3$
для того, чтобы найти частное от деления многочлен $r(x)$ на два многочлена.
Сперва я найду частное от деления многочлена
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
на многочлен
\ShowEq{p=x-i}k

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-j-k)}
Пусть
\ShowEq{p=x-i}k
\ShowEq{r=(x-j)(x-k)(x-j-k)}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q2=x2 ox 1}
Тогда
\ShowEq{s2=r-.p. 5}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=... 5}
Равенство
\ShowEq{s1=s2-.p. 5}
является следствием равенств
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5}.
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q0=... 5}
Равенство
\ShowEq{s0=s1-.p. 5}
является следствием равенств
\EqRef{s1=s2-.p. 5},
\EqRef{q0=... 5}.
Равенство
\ShowEq{r=s0+q1+q2 5}
является следствием равенств
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5},
\EqRef{q0=... 5},
\EqRef{s0=s1-.p. 5}.
\end{\ExampleStyle}

Частное
\ShowEq{q=q1+q2 5}
от деления многочлена
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
на многочлен
\ShowEq{p=x-i}k
является тензором зависящим от $x$,
а не многочленом.
Поэтому мы не можем применить теорему
\RefTheorem{r=+q circ (x-a)}.
}

\DefQuestion{how to select factor in the tensor}
{
Нетрудно убедиться, что
\ShowEq{q1+q2 5 x=j}
Поэтому возникает вопрос как выделить в тензоре
\DrawEq{q1+q2 5 x}1
множитель $x-j$.
}

\DefExample{select factor in the tensor}
{
Один из возможных ответов на вопрос
\RefQuestion{how to select factor in the tensor}
состоит в преобразовании
\ShowEq{q1+q2 5 x,1}
Рассмотрим многочлен
\DrawEq{q1+q2 5 x,3}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 7}
Теперь мы положим
\ShowEq{q0= 7}
Тогда
\ShowEq{s0=s-.p. 7}
Равенство
\ShowEq{r=x2... 7}
является следствием равенств
\EqRef{s1=r-.p. 7},
\EqRef{s0=s-.p. 7}.
Равенство
\ShowEq{q1+q2 5 x,2}
является следствием равенств
\EqRef{q1+q2 5 x,1},
\EqRef{r=x2... 7}.
}

\AddEq{remark: select factor in the tensor}
{
Мы видим, что частное в примере
\RefExample{select factor in the tensor}
является $H^{3\otimes}$\Hyph числом.
}

\DefExample{factorization as bilinear map}
{
Равенство
\ShowEq{r= 8}
является следствием равенств
\EqRef{r=s0+q1+q2 5},
\EqRef{q1+q2 5 x,2}.
}

\DefQuestion{factorization as bilinear map}
{
Равенство
\EqRef{r= 8}
является ответом на вопрос
\RefQuestion{how to select factor in the tensor}.
Мы видим, что разложение многочлена $r(x)$
является билинейным отображением многочленов
$x-j$, $x-k$.
Однако этот ответ не полный.
Согласно замечанию
\RefRemark{monomial of power k},
представление
\EqRef{r=+q circ p}
многочлена не единственно.
Остаётся открытым вопрос о выборе множителей и их порядке.
В то же время существует связь между различными представлениями многочлена
в виде произведения множителей.
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теорем
\RefTheorem{action of ring of rational integers in Abelian group},
\RefTheorem{Abelian group is free}
и определения
\RefDefinition{module over commutative ring}
следует, что свободная абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Пусть произведение в алгебре
\AoxA H
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{RH}
Представление
\DrawEq[RH]{h:AoxA->L(A)}H
$R$\Hyph алгебры
\AoxA H
в абелевой группе
\ShowEq{L(A->B)}RHH,
определённое равенством
\DrawEq[RH]{representation AA in LA}{RH}
является левым \BoxB{H}модулем.
Если мы положим $g=E$,
где
\ShowEq{product in algebra AA 3}RHE
- тождественное отображение,
то мы можем отождествить линейное отображение
\ShowEq{f: A->B}fHH{}
алгебры кватернионов и тензор
\DrawEq{linear map f, basis E}1
опираясь на равенство
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
Теорема является следствием утверждения
что отображение
\ShowEq{Eox=x}
порождает любое линейное отображение алгебры кватернионов
}

\DefDefinition{square root}
{
Решение
\ShowEq{square root}
уравнения
\DrawEq{x2=a}{root}
в $D$\Hyph алгебре $A$
называется
\AddIndex{квадратным корнем}{square root}
$A$\Hyph числа $a$.
}

\DefDefinition{polynomial*polynomial}
{
Билинейное отображение
\ShowEq{polynomial*polynomial}
определено равенством
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
Для любых тензоров
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
произведение однородных многочленов
\ShowEq{polynomials a o x,b o x}
определено равенством
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Пусть $H$ - алгебра кватернионов и $a$ - $H$\Hyph число.
\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{Re sqrt a ne 0}
то уравнение
\DrawEq{x2=a}{}
имеет корни
\ShowEq{x=x12}
такие, что
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Если $a=0$, то уравнение
\DrawEq{x2=a}{}
имеет корень $x=0$ кратности $2$.
\labelItem{a=0}
\item
Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней таких, что
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
Полилинейное отображение $D$\Hyph алгебры $A$
\ShowEq{f:A->B}f{A^n}A
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Обозначим
\ShowEq{set polylinear maps An}DAA
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$.
}

\DefRemark{monomial of power k}
{
В теореме
\RefTheorem{monomial of power k}
я рассмотрел рекурсивное представление одночлена в ассоциативной $D$\Hyph алгебре.
Так как скобки в произведении
я могу расставить произвольно,
то в ассоциативной $D$\Hyph алгебре
рекурсивное представление одночлена неоднозначно.
Например, одночлен $ax^2bxcx^3d$
может быть записан в любой из следующих форм
\ShowEq{ax^2bxcx^3d}
Я выбрал равенство
\EqRef{monomial of power k, F=1}
как самое простое для алгоритма деления многочленов.
}

\DefTheorem{monomial of power k}
{
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над ассоциативной $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
где $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
Мы докажем утверждение теоремы индукцией по степени
$n$ одночлена.

Пусть $n=0$.
Так как одночлен $p_0(x)$ является константой,
то мы получаем утверждение
\RefItem{monomial of power 0}.

Пусть $n=k$. Последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.
}

\DefTheorem{r=+q circ p}
{
Пусть
\ShowEq{p=p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
}

\DefDefinition{linear map of A vector space}
{
Пусть $A$ - $D$\Hyph алгебра с делением.
Пусть $V$, $W$ - левые векторные пространства над $D$\Hyph алгеброй $A$.
Линейное отображение
\ShowEq{f:A->B}fVW
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{линейным отображением}{linear map}
левого $A$\Hyph векторного пространства $V$
в левое $A$\Hyph векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, VW module}
множество линейных отображений
левого $A$\Hyph векторного пространства $V$
в левое $A$\Hyph векторное пространство $W$.
}

\DefDefinition{component of linear map, basis E}
{
Выражение
\ShowEq{component of linear map, basis E}
в равенстве
\eqRef{linear map f, basis E}1
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Представление
\DrawEq[DA]{h:AoxA->L(A)}{}
$D$\Hyph алгебры
\AoxA A
в модуле
\ShowEq{L(A->B)}DAA,
определённое равенством
\DrawEq[DA]{representation AA in LA}{}
позволяет отождествить тензор
\ShowEq{d in AxoA}A
с линейным отображением
\ShowEq{product in algebra AA 2}DA{\delta},
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}{\delta}
имеет вид
\ShowEq{a ox b c=}
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Отображения сопряжения
имеют
стандартное представление
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
Согласно равенству
\EqRef{#2x= #1},
отображение сопряжения
\ShowEq{Map of Conjugation}{#2}
имеет матрицу
\ShowEq{#1. matrix I#2}
Равенство
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
является следствием равенств
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of algebra and ring}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с единицей \(1_A\).
Если мы отождествим \(D\)\Hyph число \(d\)
и \(A\)\Hyph число \(d\,1_A\),
то мы утверждаем, что кольцо \(D\) является подалгеброй
алгебры $A$ и
\ShowEq{D in Z(A)}

%%
Если $D$\Hyph алгебра $A$ имеет единицу, то существует
изоморфизм $f$ кольца $D$ в центр алгебры $A$.
}

\DefProof{unit of algebra and ring}
{
Пусть
\ShowEq{d12 in D}
\StartLabelItem
\begin{enumerate}
\item
Согласно утверждению
\RefItem{distributive law, module},
\ShowEq{d1+d2 in A}
Следовательно, сумма \(D\)\Hyph чисел
\(d_1\) и \(d_2\)
совпадает с суммой \(A\)\Hyph чисел
\(d_1\) и \(d_2\).
\item
Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{d1 d2 in A}
Следовательно, произведение \(D\)\Hyph чисел
\(d_1\) и \(d_2\)
совпадает с произведением \(A\)\Hyph чисел
\(d_1\) и \(d_2\).
\end{enumerate}
Из утверждений
\RefItem{d1+d2 in A},
\RefItem{d1 d2 in A}
следует, что кольцо \(D\) является подалгеброй
алгебры $A$.

Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
Из равенства
\EqRef{ad=da in A}
следует, что
\ShowEq{D in Z(A)}

%%
Пусть $e\in A$ - единица алгебры $A$.
Положим $f\circ a=ae$.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
Произведение в алгебре $A$ дистрибутивно по отношению к сложению
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{=module}
\ShowEq{=DD}
Линейное отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
%\ShowEq{D ab in A, d in D}RH
\ShowEq{D ab in A, d in D}DA
Обозначим
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
множество линейных отображений
%алгебры кватернионов $H$.
$D$\Hyph алгебры $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Копроизведение в категории \SideRu\TO $\Base$\Hyph \VectorsSetRuB называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
для прямой суммы \SideRu\TO $\Base$\Hyph \VectorsSetRuB $\Module$ и $\ModuleA$.
}{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\AddEq{theorem: direct sum of D modules}
{
\begin{ShadedTheorem}
\labelTheorem{direct sum of \SideWS \Base-\VectorsSetNS}
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\algebrab $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph модулей
\ShowEq{o+Ai}{\Module}
\end{ShadedTheorem}
}

\DefProof{direct sum of D modules}
{
Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRu\To $\Base$\Hyph модуль $V$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\DefProof{cr-power, 1}
{
Равенство
\ShowEq{cr-power, 1 1}
является следствием равенств
\EqRef{cr power, 0},
\EqRef{cr-power, n}.
Равенство
\EqRef{cr-power, 1}
является следствием равенства
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
Равенство
\ShowEq{rc-power, 1 1}
является следствием равенств
\EqRef{rc power, 0},
\EqRef{rc-power, n}.
Равенство
\EqRef{rc-power, 1}
является следствием равенства
\EqRef{rc-power, 1 1}.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Если
\ShowEq{c in ZAa}ab,
то
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Пусть
\ShowEq{c in ZAa}ab.
Равенство
\DrawEq{ab=ba}Z
является следствием утверждения
\eqRef{c in S=>bc=cb}{Z(A,b)}.
Теорема является следстием равенства
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Если
\ShowEq{c in ZAa}ab{}
и
\ShowEq{c in ZA}c
то
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
Равенство
\ShowEq{a(bc)=...=(bc)a}
является следствием определений
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Теоремя является следствием равенства
\EqRef{a(bc)=...=(bc)a}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $b\in A$ существует подалгебра
\ShowEq{center of A number}
$D$\Hyph алгебры $A$ такая, что
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph алгебра
\ShowEq{center Ac}{}
называется
\AddIndex{центром $A$\Hyph числа}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
Подмножество
\ShowEq{center Ac}{}
не пусто так как
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Пусть
\ShowEq{d in D c in S 12}
Тогда
\ShowEq{dcb=bdc}
Откуда следует
\ShowEq{dc in S}
Следовательно, множество
\ShowEq{center Ac}{}
является $D$\Hyph модулем.

Пусть
\ShowEq{c in ZAb}
Тогда
\ShowEq{c1c2 in ZAb}
Из равенства
\EqRef{c1c2 in ZAb}
следует, что
\ShowEq{c1 c2 in ZAb}
Следовательно, $D$\Hyph модуль
\ShowEq{center Ac}{}
является $D$\Hyph алгеброй.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Для любого множества $B$
множество отображений $A^B$ является абелевой группой относительно операции
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
Теорема является следствием определений
\RefDefinition{module over commutative ring},
\RefDefinition{algebra over ring}.
}

\AddEq{theorem: definition of module over commutative ring}
{
\begin{ShadedTheorem}
\labelTheorem{definition of module}
Элементы $D$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закону ассоциативности}{associative law}
\DrawEq{associative law, module}2
\item 
\labelItem{distributive law, module}
\AddIndex{закону дистрибутивности}{distributive law}
\DrawEq{distributive law, module, 1}1
\DrawEq{distributive law, module, 2}1
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, D-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
\end{ShadedTheorem}
}

\AddEq{definition: module over algebra}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS \VectorSet over algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра \DivisionRuNS.
Эффективное \SideRu востороннее представление
\ShowEq{\SideWS A->*V}
$D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{\SideRu вым \VectorSetRuE}{\SideWS \VectorSetNS}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph \VectorSetRuA $V$ является
\AddIndex{\SideRu вым $A$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\ShowEq{\SideWS AV->V}
порождённое \SideRu восторонним представлением
\ShowEq{AV->V to \SideWS product}
называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
вектора на скаляр.
\end{ShadedDefinition}
}

\AddEq{theorem: module over algebra}
{
\begin{ShadedTheorem}
\labelTheorem{\SideWS module over algebra}
Следующая диаграмма представлений описывает \SideRu\To $\Base$\Hyph модуль $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
\end{ShadedTheorem}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\def\Temp{}
\ifx\SideNS\Temp
\RefDefinition{module over commutative ring}
и теоремы
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefDefinition{\SideWS module over algebra}
%и следствия
%\RefCorollary{Free Algebra over Ring}.
и теоремы
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
}
\end{ShadedLemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\RefDefinition{linear map from A1 to A2, commutative module},
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
{\it
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
}
\end{ShadedLemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лем
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\AddEq{theorem: A module -> algebra is associative}
{
\begin{ShadedTheorem}
\labelTheorem{\SideWS A module -> algebra is associative}
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
\end{ShadedTheorem}
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\AddEq{theorem: definition of A module}
{
\begin{ShadedTheorem}
\labelTheorem{definition of \SideWS module}
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\EqRef{diagram of representations, \SideWS module},
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnote{
Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.
}
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\algebrab $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
Если \algebrac $\Base$ имеет единицу, то
\ShowEq{A1=A unital extension}
Если \algebrac $\Base$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}
В противном случае
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
\algebraD $\Base$ является \SideRu\What идеалом \algebrab $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \algebrab $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
\end{ShadedTheorem}
}

\AddEq{theorem: definition of A module, property}
{
\begin{ShadedTheorem}
\labelTheorem{definition of \SideWS module, property}
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{p,q in \Base 1, v,w in V}
\end{ShadedTheorem}
}

\AddEq{proof: definition of A module}
{%
{\sc Доказательство теорем
\RefTheorem{definition of \SideWS module},
\RefTheorem{definition of \SideWS module, property}.}
Пусть $v\in V$.

\begin{ShadedLemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{ShadedLemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{\SideWS module over algebra}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \algebrab $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
\RefTheorem{definition of \SideWS module, property},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\AddEq{definition: submodule}
{
\begin{ShadedDefinition}
\labelDefinition{submodule, \SideWS module}
Подпредставление $\Base$\Hyph \SideRu\From модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu\From $\Base$\Hyph модуля $V$.
\qed
\end{ShadedDefinition}
}

\AddEq{theorem: submodule}
{
\begin{ShadedTheorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu\From $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi}v
принадлежат подмодулю $V'$ \SideRu\From $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi}v
принадлежит подмодулю $V'$.
\end{ShadedTheorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определений
\RefDefinition{\SideWS linear combination of vectors},
\RefDefinition{submodule, \SideWS module}.
}

\AddEq{theorem: set of vectors generated by set of vectors}
{
\begin{ShadedTheorem}
\labelTheorem{set of vectors generated by set of vectors, \SideWS module}
Пусть $V$ - \SideRu\To $\Base$\Hyph модуль.
Множество векторов, порождённое множеством векторов
\ShowEq{vi V},
имеет вид\,\footnotemark
\ShowEq{w=sum vi, \SideWS module}
\end{ShadedTheorem}
\footnotetext{\,
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
Согласно теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
мы должны доказать следующие утверждения:
\ShowEq{vectors generated by set of vectors}

\begin{itemize}
\item
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}{\Base_{(1)}}
Тогда
\ShowEq{vk=sum vi, \SideWS module}
Утверждение
\RefItem{\SideWS module, vk in Jv}
следует из
\EqRef{w=sum vi, \SideWS module},
\EqRef{vk=sum vi, \SideWS module}.
\item
Утверждение
\RefItem{\SideWS module, cvk in Jv}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{definition of \SideWS module}
и утверждения
\RefItem{\SideWS module, vk in Jv}.
\item
Так как $V$ является абелевой группой,
то утверждение
\RefItem{\SideWS module, sum cvk in Jv}
следует из утверждения
\RefItem{\SideWS module, cvk in Jv}
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
и теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.
\else
и теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{structure of Abelian group}.
\fi
\item
Пусть
\ShowEq{w12 in Jv}wv
Так как $V$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\DrawEq{w1+w2 in V}{\SideNS}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{gi12}w
такие, что
\DrawEq[w]{w12= \SideNS}{module}
где множества
\DrawEq[w]{|ci12 ne 0|}{\SideWS module}
конечны.
Так как $V$ является абелевой группой,
то из равенства
\eqRef{w12= \SideNS}{module}
следует, что
\DrawEq[w]{w1+w2= \SideNS}{module}
Равенство
\DrawEq[w]{w1+w2= 1 \SideNS}{module}
является следствием равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w1+w2= \SideNS}{module}.
Из равенства
\eqRef{|ci12 ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}w
конечно.
\item
Пусть
\ShowEq{w in Jv}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{(1)}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{set au vi}w
такие, что
\ShowEq{w= \SideWS module}
где
\DrawEq{|wi ne 0|}{\SideWS module}
Из равенства
\EqRef{w= \SideWS module}
следует, что
\ShowEq{aw= \SideWS module}
Из утверждения
\eqRef{|wi ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |awi ne 0|}
конечно.
\end{itemize}
Из равенств
\eqRef{w1+w2 in V}{\SideNS},
\eqRef{w1+w2= 1 \SideNS}{module},
\EqRef{aw in Xk \SideWS module},
\EqRef{aw= \SideWS module}
следует, что
\ShowEq{Xk+1 in Jv}
}

\AddEq{theorem: d in D->d in D1}
{
\begin{ShadedTheorem}
\labelTheorem{d in D->d in D1, \SideWS module}
Отображение
\ShowEq{f:a in A->b in B}{I_{(1)}}d{\Base}{d+0}{\Base_{(1)}}
является гомоморфизмом \algebrab $\Base$
в \algebrad $\Base_{(1)}$.
\end{ShadedTheorem}
}

\DefProof{d in D->d in D1}
{
Равенство
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)+(b+m)=}{\SideWS module}.
Равенство
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
Теорема является следствием равенств
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}.
}

\AddEq{theorem: da in DA->da in D1A}
{
\begin{ShadedTheorem}
\labelTheorem{da in DA->da in D1A, \SideWS module}
Отображение
\ShowEq{da in DA->da in D1A}
является морфизмом \SideRu\From $\Base$\Hyph модуля $V$
в \SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
\end{ShadedTheorem}
}

\DefProof{da in DA->da in D1A}
{
Равенство
\ShowEq{da in DA->da in D1A 1, \SideWS module}
является следствием теоремы
\RefTheorem{d in D->d in D1, \SideWS module}.
Теорема является следствием равенства
\EqRef{da in DA->da in D1A 1, \SideWS module}
и определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\AddEq{convention: da in DA->da in D1A}
{
\begin{convention}
\labelConvention{da in DA->da in D1A, \SideWS module}
Согласно теоремам
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem{da in DA->da in D1A, \SideWS module},
множество слов, порождающих
\SideRu\To $\Base$\Hyph модуль $V$,
совпадает с множество слов, порождающих
\SideRu\To $\Base_{(1)}$\Hyph модуль $V$.
Поэтому, не нарушая общности,
мы будем предполагать, что \algebrac $\Base$
имеет единицу.
\qed
\end{convention}
}

\DefLabeledDefinition{linear combination of vectors}{\SideWS}
{
Пусть $\Module$ - \SideRu вое $\Base$\Hyph \VectorSetRuA.% столбцов.
Пусть
\ShowEq{vi V}{}
- множество векторов.
\ShowEq{\SideWS linear combination}%
Выражение
\ShowEq{A linear combination =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{vi}
Вектор
\ShowEq{w=wi vi\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{vi}
}

\AddEq{definition: generating set of module}
{
\begin{ShadedDefinition}
\labelDefinition{generating set of \SideWS module}
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $D$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
\qed
\end{ShadedDefinition}
}

\AddEq{remark: generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\AddEq{remark: basis of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\AddEq{definition: basis of module}
{
\begin{ShadedDefinition}
\labelDefinition{basis of \SideWS module}
Если множество $X\subset V$ является множеством образующих
\SideRu\From $D$\Hyph модуля $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $D$\Hyph модуля $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $D$\Hyph модуль $V$, то такое множество $X$ называется
\AddIndex{базисом}{basis} \SideRu\From $D$\Hyph модуля $V$.
\qed
\end{ShadedDefinition}
}

\AddEq{theorem: linearly depends on rest of vectors}
{
\begin{ShadedTheorem}
\labelTheorem{linearly depends on rest of vectors, \SideWS module}
Пусть $\Base$ - \Algebra.
Если уравнение
\ShowEq{\SideWS wi vi=0}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0},
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{ShadedTheorem}
}

\AddEq{proof: linearly depends on rest of vectors}
{
\begin{proof}
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}v
и определения
\RefDefinition{\SideWS linear combination of vectors}.
\end{proof}
}

\AddEq{remark: 0=0vi}
{
Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{\SideWS 0=0vi}
}

\AddEq{remark: scalars and vectors as matrix}
{
Представим множество $\Base$\Hyph чисел
\ShowEq{set au vi}w
в виде матрицы
\ShowEq{column vector w=wi}wn
Представим множество векторов
\ShowEq{set vi}v
в виде матрицы
\ShowEq{row vector w=wi}vn
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=wi vi\SideNS}
в виде
\ShowEq{w=w cr v}
}

\AddEq{definition: linearly independent vectors}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS linearly independent vectors}
Множество векторов\,\footnote{
Я следую определению в
\citeBib{Serge Lang}, страница 100.}
\ShowEq{set vi}v
\SideRu\From $\Base$\Hyph модуля $V$
\AddIndex{линейно независимо}{linearly independent set},
если $w=0$ следует из уравнения
\ShowEq{\SideWS wi vi=0}
В противном случае, множество векторов
\ShowEq{set vi}v
\AddIndex{линейно зависимо}{linearly dependent set}.
\qed
\end{ShadedDefinition}
}

\AddEq{theorem: basis of module}
{
\begin{ShadedTheorem}
\labelTheorem{basis of \SideWS module}
Множество векторов
\ShowEq{basis for module over algebra}
является базисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e_{\gii}$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
\end{ShadedTheorem}
}

\DefProof{basis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определению
\RefDefinition{\SideWS linear combination of vectors},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\RefDefinition{generating set of \SideWS module}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество $\Basis e$ является базисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: division algebra, basis}
{
\begin{ShadedTheorem}
\labelTheorem{division algebra, \SideWS basis}
Пусть $\Base$ - \AlgebraRuNS\DivisionRuNS.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu вого $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы $e_{\gii}$ линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{ShadedTheorem}
}

\DefProof{division algebra, basis}
{
Пусть множество векторов
\ShowEq{set vi}e
линейно зависимо. Тогда в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}.
Согласно теореме
\RefTheorem{linearly depends on rest of vectors, \SideWS module},
вектор $e_{\gij}$
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество векторов
\ShowEq{set vi}e
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{set vi}e
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{set vi}e
то множество векторов $v$,
\ShowEq{set vi}e
не является линейно независимым.
}

\DefConvention{unit of algebra in basis}
{
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
}

\DefDefinition{linear map from D1 A1 to D2 A2, module}
{
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
$D_1$\Hyph модуля $A_1$
в $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}

\DefTheorem{algebra A2 representation in LA}
{
Пусть $A_1$ и $A_2$ являются $D$\Hyph алгебрами.
Пусть произведение в алгебре \AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{A2}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnote{
Определение представления
$\Omega$\Hyph алгебры дано в определении
\ShowEq{ref definition: representation of algebra}.
}
алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
}

\ifx\texFuture\Defined
\AddEq{linear map from D1 A1 to D2 A2, module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map from D1 A1 to D2 A2, \SideNS module}
{\it
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
\SideRu\From $D_1$\Hyph модуля $A_1$
в \SideRu\To $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu\From $D_1$\Hyph модуля $A_1$ в \SideRu\To $D_2$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}
\qed
\end{ShadedDefinition}
}
\fi

\DefDefinition{homomorphism from A1 to A2, D algebra}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
называется
\AddIndex{гомоморфизмом}{homomorphism}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Обозначим
\ShowEq{set homomorphisms, D algebra}
множество гомоморфизмов
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
}

\DefTheorem{homomorphism from A1 to A2, D algebra}
{
Гомоморфизм
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D algebra}
\DrawEq[{}fa]{f(da)=h... module}{D algebra}
\ShowEq{fab=fa fb}
\ShowEq{D ab in A, d in D}D{A_1}
}

\DefProof{homomorphism from A1 to A2, D algebra}
{
Из определений
\RefDefinition{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{algebra over ring}
следует, что
отображение $f$ является линейным отображением $D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$ (равенства
\eqRef{f(a+b)=...}{D algebra},
\eqRef{f(da)=h... module}{D algebra})
которое сохраняет произведение
(pавенство
\EqRef{fab=fa fb}).
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
Если произведение в $D$\Hyph алгебре $A$ имеет единичный элемент,
то $D$\Hyph алгебра $A$ называется
\AddIndex{унитальной алгеброй}{unital algebra}.\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение унитальной алгебры также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph алгебра \(A\) называется
\AddIndex{алгеброй с делением}{division algebra},
если для любого \(A\)\Hyph числа \(a\ne 0\)
существует \(A\)\Hyph число \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Из утверждения
\ShowEq{ab=ac a ne 0}
следует, что $b=c$.
}

\DefProof{division algebra}
{
Равенство
\ShowEq{ab=ac a ne 0 1}
является следствием утверждения
\EqRef{ab=ac a ne 0 1}.
}

\DefDefinition{linear map from A1 to A2, commutative module}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
Множество
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Пусть $A$ - нормированный $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - нормированный $D$\Hyph модуль с нормой $|y|_B$.
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}D{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\ShowEq{f()},
\ShowEq{g()}.
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnotemark
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\ShowEq{g()}{}
на $B_1$\Hyph число
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
}

\DefDefinition{symmetric polylinear map}
{
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$a_i=a_{i+1}$
хотя бы для одного\,\footnotemark
\ShowEq{1<=i<n}
}{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}

\DefTheorem[3]{alternation of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\ShowEq{[f]},
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefDefinition{coordinates of vector 2016}
{
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Матрица $\Base$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\fi
}

\AddEq{definition: coordinates of vector}
{
\begin{ShadedDefinition}
\labelDefinition{coordinates of vector, \SideWS module}
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
Матрица $\Base$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\qed
\end{ShadedDefinition}
}

\AddEq{theorem: linear dependence between vectors of basis}
{
\begin{ShadedTheorem}
\labelTheorem{linear dependence between vectors of basis, \SideWS module}
Пусть $\Base$ - \algebra.
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$.
Пусть
\DrawEq[w]{c*e=0, \SideWS module}{1}
линейная зависимость векторов базиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base$\Hyph число
\ShowEq{wi i in I}
не имеет обратного элемента
в \algebraa $\Base$.
\item
Множество $\Base'$ матриц
\ShowEq{w=wi i in I}
порождает \SideRu\To $\Base$\Hyph модуль $\Base'$.
\end{enumerate}
\end{ShadedTheorem}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{w=wi i in I}
такая, что равенство
\eqRef{c*e=0, \SideWS module}{1}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Если мы положим, что $\Base$\Hyph число $c^{\gij}$
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}e
является следствием равенства
\eqRef{c*e=0, \SideWS module}{1}.
Следовательно вектор $e_{\gij}$
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является базисом.
Следовательно, наше предположение неверно,
и $\Base$\Hyph число $c^{\gij}$ не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[b]{c*e=0, \SideWS module}{}
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\AddEq{theorem: coordinates of vector with linear dependence}
{
\begin{ShadedTheorem}
\labelTheorem{coordinates of vector with linear dependence, \SideWS module}
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет базис $\Basis e$ такой, что в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{2}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{w=wi i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
\end{ShadedTheorem}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{c*e=0, \SideWS module}{2}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно базиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{c*e=0, \SideWS module}{2},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.
}

\AddEq{definition: free module over ring}
{
\begin{ShadedDefinition}
\labelDefinition{free \SideWS module}
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnote{
Я следую
определению в \citeBib{Serge Lang}, страница 103.}
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис
и векторы базиса линейно независимы.
\qed
\end{ShadedDefinition}
}

\AddEq{theorem: coordinates of vector of free module}
{
\begin{ShadedTheorem}
\labelTheorem{coordinates of vector of free \SideWS module}
Координаты вектора $v\in V$ относительно базиса $\Basis e$
свободного \SideRu\From $\Base$\Hyph модуля $V$
определены однозначно.
\end{ShadedTheorem}
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\RefTheorem{coordinates of vector with linear dependence, \SideWS module}
и определений
\RefDefinition{\SideWS linearly independent vectors},
\RefDefinition{free \SideWS module}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnotemark
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}DAA{}
имеет следующее разложение
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA,
то согласно определению
\RefDefinition{free module},
существует разложение
\DrawEq[A]{expansion of linear map with respect to basis}A
линейного отображения $f$ относительно базиса $\Basis F$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
Равенство
\eqRef{map f generated by basis F}{associative algebra}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A->A, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefConvention{av=sum av convention}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av convention}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefTheorem{effective representation of the ring}
{
%Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
}

\DefProof{effective representation of the ring}
{
Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенств
\EqRef{sum of transformations of Abelian group, 1},
\EqRef{representation of ring, 1}
следует, что
\ShowEq{representation of ring, 2}
Равенство
\ShowEq{f(a-b)=0}
является следствием равенств
\EqRef{0ov=0},
\EqRef{representation of ring, 2}.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
}

\DefTheorem{Representation of ring f(0)=v0}
{
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
удовлетворяет равенству
\ShowEq{f(0)=v0}
где
\ShowEq{0:A->A}
отображение такое, что
\ShowEq{0ov=0}
}

\DefProof{Representation of ring f(0)=v0}
{
Равенство
\ShowEq{fa=fa+f0}
является следствием равенства
\EqRef{sum of transformations of Abelian group, 1}.
Равенство
\ShowEq{f0x=0}
является следствием равенства
\EqRef{fa=fa+f0}.
Равенство
\EqRef{0ov=0}
является следствием равенств
\EqRef{f(0)=v0},
\EqRef{f0x=0}.
}

\AddEq{remark: sum of transformations of Abelian group}
{
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление
\ShowEq{f:A->*B}fDA
кольца $D$ в абелевой группе $A$, мы полагаем
\ShowEq{f(a)+f(b)=}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом кольца $D$.
Следовательно
\ShowEq{f(a+b)=f(a)+f(b)}
Равенство
\ShowEq{sum of transformations of Abelian group, 1}
является следствием равенств
\EqRef{f(a)+f(b)=},
\EqRef{f(a+b)=f(a)+f(b)}.
}

\AddEq{definition: -side product}
{
%\begin{ShadedDefinition}
%\labelDefinition{\SideNS-side product}
Билинейное отображение
\ShowEq{\SideWS AV->V}
порождённое \SideRu восторонним представлением $g_{2,3}$ называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
вектора на скаляр.
%\qed
%\end{ShadedDefinition}
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
Согласно \citeBib{math.QA-0208146},
\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=3}{page 3}
у нас нет определения
детерминанта в случае алгебры с делением.\,\footnote{
В алгебре кватернионов профессор Кирчей
пользуется двойным определителем
(смотри определение в разделе
\citeBib{1812.03397}\Hyph 2.2)
для решения системы линейных уравнений
и для решения задачи о собственных значениях
(смотри раздел
\citeBib{1812.03397}\Hyph 2.5).
Я ограничился рассмотрением квазидетерминантов,
так как меня интересует более широкий класс алгебр.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn

\,

\citeBib{1812.03397}
Ivan Kyrchei,
Linear differential systems over the quaternion skew field,
eprint \href{http://arxiv.org/abs/1812.03397}{arXiv:1812.03397} (2018)
\fi
}
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении
\RefDefinition{RC-quasideterminant},
я следую определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn

\,

\citeBib{math.QA-0208146}
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)

\,
\fi
}

\DefConvention{we use separate color for index of element}
{
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\AddEq{theorem: direct sum of n D modules}
{
\begin{ShadedTheorem}
\labelTheorem{direct sum of n \SideWS \Base-\VectorsSetNS}
Прямая сумма \SideRu вых $\Base$\Hyph \VectorsSetRuB
\ShowEq{a1n}{\Module}n{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}{\Module}
\end{ShadedTheorem}
}

\AddEq{theorem: foa=fi ai}
{
\begin{ShadedTheorem}
\labelTheorem{foa=fi ai, \SideWS \Base-\VectorsSetNS}
Пусть
\ShowEq{A 1n}{\Module}n{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
Представим $\VNumber$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\ShowEq{a=(a1.n col)}{\VNumber}n
Представим линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
как вектор строку
\ShowEq{a=(a1.n row)}fn
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Тогда значение отображения $f$ в $\Module$\Hyph числе $\VNumber$
можно представить как произведение матриц
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
\end{ShadedTheorem}
}

\DefProof{foa=fi ai}
{
Теорема является следствием определения
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\AddEq{theorem: foa=fi a}
{
\begin{ShadedTheorem}
\labelTheorem{foa=fi a, \SideWS \Base-\VectorsSetNS}
Пусть
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\ShowEq{a=(a1.n col)}{\VNumberA}m
Тогда линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
имеет представление как вектор столбец отображений
\ShowEq{a=(a1.n col)}fm
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
\end{ShadedTheorem}
}

\DefProof{foa=fi a}
{
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Выражение
$\ShowSymbol{standard component of tensor}{}$
определено однозначно и называется
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
}

\AddEq{theorem: map of direct sum of modules}
{
\begin{ShadedTheorem}
\labelTheorem{map of direct sum of modules, \SideWS \Base-\VectorsSetNS}
Пусть
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\Module$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\ShowEq{a=(a1.n col)}{\VNumber}n
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\ShowEq{a=(a1.n col)}{\VNumberA}m
Тогда линейное отображение $f$
имеет представление как матрица отображений
\ShowEq{a=(a11.nm matrix)}fnm
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
Отображение
\ShowEq{fij:->}{\Module}{\ModuleA}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
\end{ShadedTheorem}
}

\DefProof{map of direct sum of modules}
{
Согласно теореме
\RefTheorem{foa=fi a, \SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
Согласно теореме
\RefTheorem{foa=fi ai, \SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $f^i_j$
с помощью \BoxB{B^i}чисел.
}

\AddEq{text: Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\AddEq{theorem: linear map of A module, coordinates}
{
\begin{ShadedTheorem}
\labelTheorem{linear map of \SideWS A module, coordinates \Base\DF\Base\DT}
\ShowEq{Let be basis of module}{\Base_\DF}iI{}{D_1}{\Base_\DF}
\ShowEq{Let be basis of module}{\Base_\DT}jJ{}{D_2}{\Base_\DT}
\ShowEq{Let be basis of module}{\Module_1}kK{\SideRu\Which}{\Base_\DF}{\Module_1}
\ShowEq{Let be basis of module}{\Module_2}lL{\SideRu\Which}{\Base_\DT}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
имеет представление
\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
\end{ShadedTheorem}
}

\DefProof{linear map of A module, coordinates}
{
Равенство
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
является следствием теоремы
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map in A module}{\SideNS}
является следствием теоремы
\RefTheorem{map of direct sum of modules}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}DA
алгебры \AOn
в модуле \LAnA,
определённое равенством
\DrawEq[DA]{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[DA]{product in algebra An 2}{DA}
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\AddEq{remark: notation for linear map}
{
Если отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$,
то, согласно определению
\RefDefinition[\RefRepresentation]{left-side representation of group},
%\RefDefinition[\RefRepresentation]{\SideNS-side representation of group},
я пользуюсь обозначением
\DrawEq{f circ a =}{}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},%, associative algebra},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\end{proof}
}
{proof: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A->B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\ShowEq{f:A->B}f{A_1}{A_2}
имеет вид
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
Множество линейных отображений
\ShowEq{vI=EI}
является базисом
левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}
и линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
$#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
\ShowEq{vI=... #1}
и $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
кватернионы, представленные строками матрицы $f$.
\ShowEq{fi=fij ej H}
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}O
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map, maps of conjugation, algebra C}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\ShowEq{f:A->B}fCC
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a...= C}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{ShadedTheorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{ShadedTheorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\AddEq{definition: linear map A module}
{
\begin{ShadedDefinition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{ShadedDefinition}
}

\AddEq{definition: homomorphism A module}
{
\begin{ShadedDefinition}
\labelDefinition{homomorphism \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for homomorphism}1
в диаграмму представлений
\ShowEq{A module diagram for homomorphism}2
называется
\AddIndex{гомоморфизмом}{homomorphism}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set homomorphisms, \SideWS A12 module}
множество гомоморфизмов
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{ShadedDefinition}
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{linear map from A1 to A2, module}
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{ShadedDefinition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\AddEq{theorem: linear map of module}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}hf
\SideRu\From $\Base_{\DF}$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_{\DT}$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnotemark
\ShowEq{property linear map \MapE}
\end{ShadedTheorem}
\footnotetext{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
рассматривается как определение.
}
}

\DefProof{linear map, DA1->DA2, module}
{
Из определений
\RefDefinition[\RefRepresentation]{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module}
следует, что
отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D }).
Равенство
\eqRef{f(da)=h... module}{\DFDT \SideWS module}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.

Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{polylinear map of modules}
и теоремы
\RefTheorem{linear map, DA1->DA2, module}.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\RefDefinition{module over commutative ring}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A->B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\AddEq{theorem: linear map of A module}
{
\begin{ShadedTheorem}
\labelTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}gf
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnotemark
\ShowEq{property linear map \MapE}
\end{ShadedTheorem}
\footnotetext{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
рассматривается как определение.
}
}

\DefProof{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map from D1 A1 to D2 A2, module}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
является следствием равенства
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{ShadedDefinition}.
}

\DefProof{linear map of A module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module}
следует, что
\begin{itemize}
\item
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{g \DFDT \SideWS module}).
\item
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Равенства
\eqRef{f(da)=h...}{g \DFDT \SideWS module},
\eqRef{f(da)=h...}{f \DFDT \SideWS module}
являются следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{ShadedDefinition}.
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\AddEq[1]{theorem: maps of conjugation antilinear}
{
\begin{ShadedTheorem}
\labelTheorem{#1 maps of conjugation antilinear}
Отображения сопряжения
\ShowEq{I... #1}
\DoVerb являются антилинейными гомоморфизмами.
\end{ShadedTheorem}
}

\DefProof{H maps of conjugation antilinear}
{
Произведение $H$\Hyph чисел
\ShowEq{H number Ea}a
и
\ShowEq{H number Ea}b
имеет вид
\DrawEq[ab]{H product aEx}{ab}
\ShowEq{H items maps of conjugation antilinear}
}

\DefProof{O maps of conjugation antilinear}
{
Произведение $O$\Hyph чисел
\ShowEq{O number Ea}a
и
\ShowEq{O number Ea}b
имеет вид
\DrawEq[ab]{O product aEx}{ab}
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A->B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}f{A_1}{A_2}
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
%существует разложение
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
Равенство
\eqRef{map f generated by basis F}{expansion}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Пусть $A$ - $D$\Hyph алгебра.
Для любого $A$\Hyph числа $a$, отображение
\ShowEq{f->ao f}
определённое равенством
\ShowEq{ao f=a f o}
является эндоморфизмом $D$\Hyph модуля
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA
является левым $A$\Hyph модулем, порождённым представлением
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A->B)}R{#1}{#1}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\AddEq [7]{Let be basis of vector space}
{%
Пусть множество векторов
\DrawEq[{#1}{#2}{#3}]{basis e of module #6}{#7}
является базисом \SideRu вого $#4$\Hyph векторного пространства $#5$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Пусть \eV{#1}
базис \SideRu вого $#2$\Hyph векторного пространства $#3$.%
}%

\AddEq [6]{Let be basis of module}
{%
Пусть
\DrawEq[{#1}{#2}{#3}]{basis e of module cols}-
базис #4 $#5$\Hyph модуля $#6$.
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в свободном #3 $#4$\Hyph модуле $#5$.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}1{}
\DrawEq [#1{1}]{va=ae1, \SideWS module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS module}
относительно базиса
\ShowEq{basis e}2{}
\DrawEq [#9{2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}2.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}1{}
и
\ShowEq{basis e}2.
}

\DefLabeledTheorem{linear map of module, coordinates}{\SideWS \DFDT module}
{
\ShowEq{Let be basis of module}1iI{}{\Base_{\DF}}{\Module_1}
\ShowEq{Let be basis of module}2jJ{}{\Base_{\DT}}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}h{\Vector f}
имеет представление
\DrawEq[f]{r2:A1->A2, \DFDT module}{1 \SideWS f}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Module}fhiI{D_2}{}b
\end{itemize}
}

\DefProof{linear map of module, coordinates}
{
Так кaк
\ShowEq{show linear map \MapE}h{\Vector f}
линейное отображение, то равенство
\ShowEq{\DFDT vb=h(e1)a \SideNS}
является следствием равенств
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module},
\eqRef{va=ae1, \SideWS module}{a \DFDT\SideWS module},
\eqRef{vb=f(va)}{a \DFDT\SideWS module}.
$\Module_2$\Hyph число
\ShowEq{f(e1) \SideNS}
имеет разложение
\DrawEq{f(e1)= \SideNS}{\DFDT}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{\DFDT vb=h(e1)a \SideNS}
и \eqRef{f(e1)= \SideNS}{\DFDT}, мы получаем
\ShowEq{\DFDT vb=a f e \SideNS}
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS f}
следует из сравнения
\eqRef{va=ae1, \SideWS module}{b \DFDT\SideWS module}
и \EqRef{\DFDT vb=a f e \SideNS} и
теоремы \RefTheorem{coordinates of vector of free \SideWS module}.
}

\AddEq{definition: algebra over ring}
{
\begin{ShadedDefinition}
\labelDefinition{algebra over ring}
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnotemark
в $A$
\DrawEq{product in D algebra}{ShadedDefinition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\end{ShadedDefinition}
\footnotetext{\,
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.
}
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\AddEq{definition: nucleus of algebra}
{
\begin{ShadedDefinition}
\labelDefinition{nucleus of algebra}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnotemark
\ShowEq{nucleus of algebra}
\end{ShadedDefinition}
\footnotetext{\,
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13
}
}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnotemark
\ShowEq{center of algebra}
}{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14.
}

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратная матрица}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратная матрица}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество однородных многочленов}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис}%
   {Basis}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество \CR собственных значений}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество \RC собственных значений}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {образ отображения}%
   {image of map}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма групп}%
   {ker group-homomorphism}%
   {K}{0}%
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {левое векторное пространство алгебры $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {левое векторное пространство отображений}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {правое векторное пространство алгебры $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {правое векторное пространстао отображений}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {векторное пространство начальных значений системы дифференциальных уравнений}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {векторное пространство решений системы дифференциальных уравнений}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {матрица Вронского}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $A$\Hyph числа}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Text.Monomial.English.tex <==
%auto-ignore
\input{Text.\BookNumber.Eq}

\section{Square Root}

\ShowDefinition{square root}

\ShowTheorem{x2=a quaternion root}
\ProofTheorem{\RefQuadratic}{x2=a quaternion root}

\begin{\TheoremStyle}
\labelTheorem{sqrt a=...1+a}
Let quaternion $a$ be a a root of the polynomial
\DrawEq{r=xx+1}{sqrt}
Then
\ShowEq{sqrt a=...1+a}
\end{\TheoremStyle}

\begin{proof}
The equality
\ShowEq{(a+1)2=2a}
follows from the statement that $a$ is a root of the polynomial
\eqRef{r=xx+1}{sqrt}.
The equality
\EqRef{sqrt a=...1+a}
follows from the equality
\EqRef{(a+1)2=2a}
and from the statement
\RefItem{Re sqrt a ne 0}.
\end{proof}

\section{Polynomial with Given Roots}

In commutative algebra, if I have two roots of polynomial
of second order, then this polynomial is unique.
The case is different in non\Hyph commutative algebra.

\begin{\TheoremStyle}
Let
\ShowEq{x1x2 in A}
\ShowEq{x1x2/=x2x1}
Then
\DrawEq[12]{p(x)=(x-x1)(x-x2)}{12}
\DrawEq[21]{p(x)=(x-x1)(x-x2)}{21}
are unequal polynomials
\ShowEq{p12 ne p21}
\end{\TheoremStyle}

\begin{proof}
Let
\ShowEq{x=x1+x2}
The equality
\DrawEq[12]{p12 x1+x2}{12}
follows from equalities
\eqRef{p(x)=(x-x1)(x-x2)}{12},
\EqRef{x=x1+x2}.
The equality
\DrawEq[21]{p12 x1+x2}{21}
follows from equalities
\eqRef{p(x)=(x-x1)(x-x2)}{21},
\EqRef{x=x1+x2}.
The statement
\EqRef{p12 ne p21}
follows from equalities
\eqRef{p12 x1+x2}{12},
\eqRef{p12 x1+x2}{21}
and from the statement
\EqRef{x1x2/=x2x1}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{p=a1p12+a2p21}
Let
\ShowEq{a12 in AoxA}.
Then the polynomial
\ShowEq{p=a1p12+a2p21}
has roots
\ShowEq{x=x1,x2}.
\end{\TheoremStyle}

\begin{proof}
The theorem follows from the statement
that polynomials $p_{12}$, $p_{21}$
have roots
\ShowEq{x=x1,x2}.
\end{proof}

\begin{\QuestionStyle}
\labelQuestion{Does polynomial have other roots}
Does polynomial
\EqRef{p=a1p12+a2p21}
have
roots which are different from values
\ShowEq{x=x1,x2}?
\end{\QuestionStyle}

\begin{\QuestionStyle}
\labelQuestion{Are there other polynomials with given roots}
Are there other polynomials
that have roots
\ShowEq{x=x1,x2}?
\end{\QuestionStyle}

It looks like the answer to the question
\RefQuestion{Are there other polynomials with given roots}
is positive.

\begin{Example}
Consider the set of polynomials
\ShowEq{p=a1 o ij+a2 o ji}
which, according to the theorem
\RefTheorem{p=a1p12+a2p21},
have roots
\ShowEq{x=i,j}
The polynomial
\DrawEq{r=xx+1}{ij}
also has roots
\ShowEq{x=i,j}
\end{Example}

\begin{\QuestionStyle}
\labelQuestion{Does polynomial belong to the set of polynomials}
Does polynomial
\eqRef{r=xx+1}{ij}
belong to the set of polynomials
\EqRef{p=a1 o ij+a2 o ji}?
\end{\QuestionStyle}

The theorem
\RefTheorem{a1 o ij+a2 o ji=xx+1}
answers the question
\RefQuestion{Does polynomial belong to the set of polynomials}.

\begin{\TheoremStyle}
\labelTheorem{a1 o ij+a2 o ji=xx+1}
There is no tensors
\ShowEq{a12 in AoxA}{}
such that
\ShowEq{a1 o ij+a2 o ji=xx+1}
\end{\TheoremStyle}

\begin{proof}
Let the theorem be not true.

\begin{Statement}
\labelStatement{there exist a12 in AoxA}
Let there exist tensors
\ShowEq{a12 in AoxA}{}
such that
the equalitiy
\EqRef{a1 o ij+a2 o ji=xx+1}
is true.
\hfill\(\odot\)
\end{Statement}

Equalities
\ShowEq{a1 o+a2 o=xx+1 xx}
\ShowEq{a1 o+a2 o=xx+1 x}
\ShowEq{a1 o+a2 o=xx+1 1}
follow from the equality
\EqRef{a1 o ij+a2 o ji=xx+1}.

Let $x=1$.
The equality
\ShowEq{a1 o+a2 o=xx+1 x x=1}
follow from equalities
\EqRef{a1 o+a2 o=xx+1 x}.

According to the theorem
\RefTheorem{sqrt a=...1+a},
there exists x such that $x^2=i$.
The equality
\DrawEq[i]{a1 o+a2 o=xx+1 (ij) x x2=}i
follows from the equality
\EqRef{a1 o+a2 o=xx+1 xx}.

According to the theorem
\RefTheorem{sqrt a=...1+a},
there exists x such that $x^2=j$.
The equality
\DrawEq[j]{a1 o+a2 o=xx+1 (ij) x x2=}j
follows from the equality
\EqRef{a1 o+a2 o=xx+1 xx}.

The equality
\ShowEq{a1 o+a2 o=xx+1 x x=1 1}
follows from equalities
\eqRef{a1 o+a2 o=xx+1 (ij) x x2=}i,
\eqRef{a1 o+a2 o=xx+1 (ij) x x2=}j
and contradicts the equality
\EqRef{a1 o+a2 o=xx+1 x x=1}.
Therefore, the statement
\RefStatement{there exist a12 in AoxA}
is not true and we proved the theorem.
\end{proof}

\section{Division with Remainder}

\begin{\DefinitionStyle}
\labelDefinition{left divisor}
\(A\)\Hyph number \(a\)
is left divisor
of \(A\)\Hyph number \(b\),
if there exists \(A\)\Hyph number \(c\)
such that
\ShowEq{ac=b}
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{right divisor}
\(A\)\Hyph number \(a\)
is right divisor
of \(A\)\Hyph number \(b\),
if there exists \(A\)\Hyph number \(c\)
such that
\DrawEq{ca=b}{def}
\end{\DefinitionStyle}

It is evident that there is
symmetry between definitions
\RefDefinition{left divisor}
and
\RefDefinition{right divisor}.
The difference between left and right divisors
is also evident
since the product is noncommutative.
However we can consider a definition
generalizing definitions
\RefDefinition{left divisor}
and
\RefDefinition{right divisor}.

\begin{\DefinitionStyle}
\labelDefinition{divisor of A number}
\(A\)\Hyph number \(a\)
is divisor
of \(A\)\Hyph number \(b\),
if there exists
\BoxB{A}number \(c\)
such that
\DrawEq[c]{c*a=b}{c}
\BoxB{A}number \(c\) is called
\AddIndex{quotient}{quotient divided by}
of \(A\)\Hyph number \(b\) divided by \(A\)\Hyph number \(a\).
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Let division in the \(D\)\Hyph algebra \(A\)
is not always defined.
\AddIndex{\(A\)\Hyph number $a$ divides \(A\)\Hyph number $b$ with remainder}
{division with remainder},
if the following equation is true
\DrawEq{c*a+f=b}{definition}
\BoxB{A}number \(c\) is called
\AddIndex{quotient}{quotient divided by}
of \(A\)\Hyph number \(b\) divided by \(A\)\Hyph number \(a\).
\(A\)\Hyph number $f$ is called
\AddIndex{remainder of the division}{remainder of the division}
of \(A\)\Hyph number \(b\) by \(A\)\Hyph number \(a\).
\end{\DefinitionStyle}

%\ShowTheorem{r=+q circ p}
%\ProofTheorem{1302.7204}{r=+q circ p}
\begin{\TheoremStyle}
\labelTheorem{r=+q circ (x-a)}
Let
\ShowEq{p=x-i}a
be polynomial of power $1$.
Let
\ShowEq{r power k}
be polynomial of power $k>0$.
Then
\ShowEq{r=+q circ p}
where
\ShowEq{qij i j}
is homogeneous polynomial of power $i$.
\end{\TheoremStyle}
\begin{proof}
Let
\ShowEq{rk=rk0 ox rkk}
According to the theorem
\RefTheorem{monomial of power k},
\ShowEq{rk xk=...}
Let
\ShowEq{qk-1 xk-1=...}
To prove the theorem,
it is enough to note that power of the polynomial
\ShowEq{sk-1=r-qk-1 p}
is less than $k$.
The equality
\ShowEq{r=sk-1+qk-1 p}
follows from the equality
\EqRef{sk-1=r-qk-1 p}.
We will apply algorithm considered in proof to the polynomial $s_{k-1}(x)$.
After a finite number of steps, we will get the polynomial $s_0$ of power $0$.
The equality
\EqRef{r=+q circ p}
follows from the equality
\EqRef{r=sk-1+qk-1 p}.
\end{proof}

The algorithm considered in the proof of the theorem
is called standard algorithm of division of polynomials.

\section{Examples of Division of Polynomials}

In following examples, we use standard algorithm of division of polynomials.

\ShowExample{r=x2-jx-xi-k p=x-i}

\ShowRemark{r=x2-jx-xi-k p=x-i}

\ShowRemark{r=x2-ix-xj+k p=x-i}

\ShowRemark{r=x2-ix-jx-k}

\ShowQuestion{r=x2-ix-jx-k}

\ShowRemark{r=x2-ix-jx-k 1}

\ShowRemark{r=x2-ix-jx-k p=x-j}

\ShowExample{r=x2-ix-jx-k p=x-j}

\section{More Questions}

\ShowRemark{r=(x-j)(x-k)(x-j-k)}

\ShowQuestion{how to select factor in the tensor}

\ShowExample{select factor in the tensor}

\ShowRemark{select factor in the tensor}

\ShowExample{factorization as bilinear map}

\ShowQuestion{factorization as bilinear map}

If the polynomial $p(x)$ has form
\ShowEq{p=p circ x}
where $p_1$ be nonsingular tensor,
then we can use the theorem
\RefTheorem{r=+q circ (x-a)}
to divide by the polynomial $p(x)$,
if we consider the equality
\ShowEq{p=p1 (x+p1- p_0)}

\begin{\QuestionStyle}
The polynomial
\DrawEq[1]{ix-xi-1}{q1}
is divisor of the polynomial
\ShowEq{(x-j)(ix-xi-1)(x-k)}
However, we cannot use the theorem
\RefTheorem{r=+q circ (x-a)}
to find quotient,
because the tensor
\ShowEq{1 ox i-i ox 1}
is singular.
Therefore, we need additional research
to solve this problem.
\end{\QuestionStyle}

\section{Division of Polynomials in Non-associative Algebra}

\begin{Remark}
In non\Hyph associative algebra,
brackets determine in what order we perform the multiplication.
So monomial can be written as follows
\ShowEq{monomial (pq)r}
\ShowEq{monomial p(qr)}
where $p$, $q$, $r$ are also monomials.
This imposes a limitation on the possibility
to divide polynomial by a polynomial.
\end{Remark}

In the example
\RefExample{r=(x-j)(x-k)(x-jl)},
I considered the polynomial $r(x)$ of power $3$
in octonion algebra.
Becaus order of factors in product is important for defining structure of tensor,
I will explicitly write brackets even when the order is evident.
For instance, since, in general,
\ShowEq{((a ox)b)x ne (a (ox b))x}
then expressions
\ShowEq{(a ox)b}
and
\ShowEq{a (ox b)}
represent different linear maps.

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-jl)}
Let
\ShowEq{p=x-i}k
\DrawEq{r=(x-j)(x-k)(x-jl)}1
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q2=x2 (ox 1)}
Then
\ShowEq{s2=r-.p. 6}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=... 6}
The equality
\ShowEq{s1=s2-.p. 6}
follows from equalities
\EqRef{s2=r-.p. 6},
\EqRef{q1=... 6}.
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q0=... 6}
The equality
\ShowEq{s0=s1-.p. 6}
follows from equalities
\EqRef{s1=s2-.p. 6},
\EqRef{q0=... 6}.
The equality
\ShowEq{r=s0+q1+q2 6}
follows from equalities
\EqRef{s2=r-.p. 6},
\EqRef{q1=... 6},
\EqRef{q0=... 6},
\EqRef{s0=s1-.p. 6}.
\end{\ExampleStyle}

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-jl) x-j}
The quotient of the polynomial
\eqRef{r=(x-j)(x-k)(x-jl)}1
divided by the polynomial
\ShowEq{p=x-i}k
has the following form
\ShowEq{q(x)=  6}

\eqRef{r=(x-j)(x-k)(x-jl)}1
\FrameEq{r=(x-j)(x-k)(x-jl) 0}

The first term of the tensor $q(x)$
has factor $x-j$.
To check if the second term has
factor $x-j$,
consider the polynomial
\ShowEq{x^2-jx-xk+i}
According to the theorem
\RefTheorem{r=+q circ (x-a)},
we set
\ShowEq{q1=x (ox 1)}
Then
\ShowEq{s1=r-.p. 8}
Now we set
\ShowEq{q0= 8}
Then
\ShowEq{s0=s-.p. 8}
The equality
\ShowEq{r1=x2-jx-xk+i 8}
follows from equalities
\EqRef{s1=r-.p. 8},
\EqRef{s0=s-.p. 8}.
\end{\ExampleStyle}

From equalities
\EqRef{q(x)=  6},
\EqRef{r1=x2-jx-xk+i 8},
it follows that the quotient of the polynomial
\eqRef{r=(x-j)(x-k)(x-jl)}1
divided by the polynomial
\ShowEq{p=x-i}k
has the following form
\ShowEq{r=(x-j)(x-k)(x-jl) q=}

\eqRef{r=(x-j)(x-k)(x-jl)}1
\FrameEq{r=(x-j)(x-k)(x-jl) 0}

Therefore, we can represent the polynomial
\eqRef{r=(x-j)(x-k)(x-jl)}1
as follows
\ShowEq{r=(x-j)(x-k)(x-jl) bilinear}


==> Text.Monomial.Eq.tex <==
%auto-ignore

\AddEq{x1x2 in A}
{
$x_1$, $x_2\in A$,
}

\AddEquation{x1x2/=x2x1}
{
x_1x_2\ne x_2x_1
}

\AddEquation{monomial p(qr)}
{
p(x)(q(x)r(x))
}

\AddEquation{rk=rk0 ox rkk}
{
r_k=r_{k.0.s}\otimes...\otimes r_{k.k.s}
}

\AddEquation{rk xk=...}
{
\begin{split}
r_k\circ x^k&=((r_{k.0.s}\otimes...\otimes r_{k.k-1.s})\circ x^{k-1})xr_{k.k.s}
\\ &=(((r_{k.0.s}\otimes...\otimes r_{k.k-1.s})\circ x^{k-1})\otimes r_{k.k.s})\circ x
\end{split}
}

\AddEquation{qk-1 xk-1=...}
{
q_{k-1}(x)=((r_{k.0.s}\otimes...\otimes r_{k.k-1.s})\circ x^{k-1})\otimes r_{k.k.s}
}

\AddEquation{sk-1=r-qk-1 p}
{
s_{k-1}(x)=r(x)-q_{k-1}(x)\circ(x-a)
}

\AddEquation{r=sk-1+qk-1 p}
{
r(x)=s_{k-1}(x)+q_{k-1}(x)\circ(x-a)
}

\AddEquation{monomial (pq)r}
{
(p(x)q(x))r(x)
}

\AddEq[2]{p(x)=(x-x1)(x-x2)}
{
p_{#1#2}(x)=(x-x_{#1})(x-x_{#2})=x^2-x_{#1}x-xx_{#2}+x_{#1}x_{#2}
}

\AddEquation{p12 ne p21}
{
p_{12}\ne p_{21}
}

\AddEq[1]{x=x1,x2}
{
$x=x_1$, $x=x_2$#1
}

\AddEq[1]{a12 in AoxA}
{
$a_1$, $a_2\in\AoxA A$#1
}

\AddEquation{sqrt a=...1+a}
{
\sqrt{a}=\pm\frac 1{\sqrt{2}}(1+a)
}

\AddEquation{(a+1)2=2a}
{
(a+1)^2=a^2+2a+1=2a
}

\AddEquation{s2=r-.p. 6}
{
\begin{split}
s_2(x)&=r(x)-q_2(x)\circ(x-k)=r(x)-((x^2)(\otimes 1))\circ(x-k)\\
&=(x^2)x-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix+kl
\\ &-(x^2)x+(x^2)k\\
&=(x^2)k-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix+kl
\end{split}
}

\AddEquation{s1=s2-.p. 6}
{
\begin{split}
s_1(x)&=s_2(x)-q_1(x)\circ(x-k)\\
&=(x^2)k-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix+kl\\
&-((x\otimes)k-(x\otimes)jl-(jx)(\otimes 1)-(xk)(\otimes 1))\circ(x-k)\\
&=(x^2)k-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix+kl\\
&-(x(x-k))k+(x(x-k))jl+(jx)(x-k)+(xk)(x-k)\\
&=(x^2)k-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix+kl\\
&-(x^2)k+(xk)k+(x^2)jl-(xk)jl+(jx)x-(jx)k+(xk)x-(xk)k\\
&=(jx)(jl-k)+ix+kl
\end{split}
}

\AddEquation{s0=s1-.p. 6}
{
\begin{split}
s_0&=s_1(x)-q_0(x)\circ(x-k)\\
&=(jx)(jl-k)+ix+kl-((j\otimes(jl-k))+i(\otimes 1))\circ(x-k)\\
&=(jx)(jl-k)+ix+kl-(j(x-k))(jl-k)-i(x-k)\\
&=(jx)(jl-k)+ix+kl-(jx-jk)(jl-k)-ix+ik\\
&=(jx)(jl-k)+ix+kl-(jx)(jl-k)+i(jl-k)-ix-j\\
&=kl+i\,jl-ik-j=0
\end{split}
}

\AddEquation{q1=... 6}
{
q_1(x)=(x\otimes)k-(x\otimes)jl-(jx)(\otimes 1)-(xk)(\otimes 1)
}

\AddEquation{q0=... 6}
{
q_0(x)=(j\otimes)(jl-k)+i(\otimes 1)
}

\AddEq{r=(x-j)(x-k)(x-jl) 0}
{
r(x)=((x-j)(x-k))(x-jl)
}

\AddEq{r=(x-j)(x-k)(x-jl)}
{
\begin{split}
r(x)&=
((x-j)(x-k))(x-jl)
=(x^2-jx-xk+i)(x-jl)\\
&=(x^2)(x-jl)
-(jx)(x-jl)
-(xk)(x-jl)
+i(x-jl)\\
&=(x^2)x-(x^2)jl
-(jx)x-(xk)x+(jx)jl+(xk)jl
+ix-i\,jl
\end{split}
}

\AddEq{r=(x-j)(x-k)(x-j-k),1}
{
\begin{align*}
r(x)&=x^3\\
&+(-1\otimes 1\otimes j-1\otimes 1\otimes k-j\otimes 1\otimes 1-1\otimes k\otimes 1)\circ x^2\\
&+(j\otimes j+j\otimes k-1\otimes i-1\otimes 1+i\otimes 1)\circ x\\
&-k+j
\end{align*}
}

\AddEquation{x^2-jx-xk+i}
{
r_1(x)=x^2-jx-xk+i
}

\AddEq{q1=x (ox 1)}
{
$q_1(x)=x(\otimes 1)$.
}

\AddEquation{s1=r-.p. 8}
{
\begin{split}
s_1(x)&=r_1(x)-(x(\otimes 1))\circ(x-j)\\
&=x^2-jx-xk+i-x(x-j)
=x^2-jx-xk+i-x^2+xj\\
&=-jx-xk+xj+i
\end{split}
}

\AddEquation{q0= 8}
{
q_0=-j(\otimes 1)-(1\otimes)k+(1\otimes)j
}

\AddEquation{r1=x2-jx-xk+i 8}
{
\begin{split}
\EqText{r_1(x)}&=s_1(x)+(x(\otimes 1))\circ(x-j)\\
&=(-j(\otimes 1)-(1\otimes)k+(1\otimes)j+x(\otimes 1))\circ(x-j)\\
&=\EqText{((1\otimes)(j-k)+(x-j)(\otimes 1))\circ(x-j)}
\end{split}
}

\AddEquation{r=(x-j)(x-k)(x-jl) q=}
{
\begin{split}
q(x)=
&=((x-j)\otimes)(k-jl)
\\
&+(((1\otimes)(j-k)+(x-j)(\otimes 1))\circ(x-j))(\otimes 1)
\\
&=(((1\otimes_1)1\otimes)(k-jl)
\\
&+((1\otimes_1)(j-k)+(x-j)(\otimes_1 1))(\otimes 1))
\circ(x-j)
\\
&=(((1\otimes_1)1\otimes)(k-jl)
\\
&+((1\otimes_1)(j-k))(\otimes 1)+((x-j)(\otimes_1 1))(\otimes 1))
\\ &\circ(x-j)
\end{split}
}

\AddEquation{((a ox)b)x ne (a (ox b))x}
{
((a\otimes)b)\circ x=(ax)b\ne a(xb)=(a(\otimes b))\circ x
}

\AddEq{(a ox)b}
{
$(a\otimes)b$
}

\AddEq{a (ox b)}
{
$a(\otimes b)$
}

\AddEq{q2=x2 (ox 1)}
{
$q_2(x)=(x^2)(\otimes 1)$.
}

\AddEquation{r=(x-j)(x-k)(x-jl) bilinear}
{
\begin{split}
r(x)
&=(((1\otimes_1)1\otimes_2)(k-jl)
\\ &+((1\otimes_1)(j-k))(\otimes_2 1)+((x-j)(\otimes_1 1))(\otimes_2 1))
\\ &\circ(x-j,x-k)
\end{split}
}

\AddEquation{s0=s-.p. 8}
{
\begin{split}
s_0&=s_1(x)-q_0\circ p(x)=s_1(x)-(-j(\otimes 1)-(1\otimes)k+(1\otimes)j)\circ(x-j)\\
&=-jx-xk+xj+i+j(x-j)+(x-j)k-(x-j)j\\
&=-jx-xk+xj+i+jx+1+xk-i-xj-1=0
\end{split}
}

\AddEquation{r=s0+q1+q2 6}
{
\begin{split}
r(x)&=s_0+(q_0+q_1(x)+q_2(x))\circ(x-k)\\
&=(
\ShowEq{r=s0+q1+q2 6 quotient}
)\circ(x-k)
\end{split}
}

\AddEq{r=s0+q1+q2 6 quotient}
{
(j\otimes)(jl-k)+i(\otimes 1)\\
&+(x\otimes)k-(x\otimes)jl-(jx)(\otimes 1)-(xk)(\otimes 1)
+(x^2)(\otimes 1)
}

\AddEquation{q(x)=  6}
{
\begin{split}
q(x)&=
\ShowEq{r=s0+q1+q2 6 quotient}
\\
&=((x-j)\otimes)(k-jl)
+(x^2-jx-xk+i)(\otimes 1)
\end{split}
}

\AddEquation{p=p1 (x+p1- p_0)}
{
p(x)=p_1\circ (x+p_1^{-1}\circ p_0)
}

\AddEquation{(x-j)(ix-xi-1)(x-k)}
{
\begin{split}
\RedText{p(x)}&=(x-j)(ix-xi-1)(x-k)\\
&=((x-j)ix-(x-j)xi-x+j)(x-k)\\
&=xix(x-k)-jix(x-k)-x^2i(x-k)\\ &+jxi(x-k)-x(x-k)+j(x-k)\\
&=xix^2-xixk+kx^2-kxk-x^2ix+x^2ik\\ &+jxix-jxik-x^2+xk+jx-jk\\
&\RedText{=(1\otimes i\otimes 1\otimes 1-1\otimes 1\otimes i\otimes 1)\circ x^3}\\
&\RedText{+(j\otimes i\otimes 1-1\otimes i\otimes k
+k\otimes 1\otimes 1-1\otimes 1\otimes j-1\otimes 1\otimes 1)\circ x^2}\\
&\RedText{+(1\otimes k+j\otimes( 1+j)\circ x+1-i}
\end{split}
}

\AddEquation{r=x2-ix-jx-k 10}
{
\begin{split}
r(x)&=-i(x-i)-j(x-i)+(x-i)i+x(x-i)\\
&=(x-i)i+(x-i-j)(x-i)
\end{split}
}

\AddEquation{r=x2-ix-jx-k qx}
{
q(x)=
\ShowEq{r=x2-ix-jx-k map}
}

\AddEq{c*a+f=b}
{
c\circ a+f=b
}

\AddEquation{a1 o+a2 o=xx+1 x x=1 1}
{
a_1\circ i+a_2\circ i+a_1\circ j+a_2\circ j=i+j
}

\AddEquation{ac=b}
{
ac=b
}

\AddEq{ca=b}
{
ca=b
}

\AddEq[1]{c*a=b}
{
#1\circ a=b
}

\AddEquation{p=a1p12+a2p21}
{
p(x)=a_1\circ p_{12}(x)+a_2\circ p_{21}(x)
}

\AddEq[2]{p12 x1+x2}
{
p_{#1#2}(x_1+x_2)=(x_1+x_2-x_{#1})(x_1+x_2-x_{#2})=x_{#2}x_{#1}
}

\AddEquation{x=x1+x2}
{
x=x_1+x_2
}


==> Text.Monomial.Russian.tex <==
%auto-ignore
\input{Text.\BookNumber.Eq}

\section{Квадратный корень}

\ShowDefinition{square root}

\ShowTheorem{x2=a quaternion root}
\ProofTheorem{\RefQuadratic}{x2=a quaternion root}

\begin{\TheoremStyle}
\labelTheorem{sqrt a=...1+a}
Пусть кватернион $a$ является корнем многочлена
\DrawEq{r=xx+1}{sqrt}
Тогда
\ShowEq{sqrt a=...1+a}
\end{\TheoremStyle}

\begin{proof}
Равенство
\ShowEq{(a+1)2=2a}
следует из утверждения, что $a$ является корнем многочлена
\eqRef{r=xx+1}{sqrt}.
Равенство
\EqRef{sqrt a=...1+a}
является следствием равенства
\EqRef{(a+1)2=2a}
и утверждения
\RefItem{Re sqrt a ne 0}.
\end{proof}

\section{Многочлен с задаными корнями}

В коммутативной алгебре, если я имею два корня многочлена
второй степени, то этот многочлен определён однозначно.
Ситуация несколько иная в некоммутативной алгебре.

\begin{\TheoremStyle}
Пусть
\ShowEq{x1x2 in A}
\ShowEq{x1x2/=x2x1}
Тогда
\DrawEq[12]{p(x)=(x-x1)(x-x2)}{12}
\DrawEq[21]{p(x)=(x-x1)(x-x2)}{21}
неравные многочлены
\ShowEq{p12 ne p21}
\end{\TheoremStyle}

\begin{proof}
Пусть
\ShowEq{x=x1+x2}
Равенство
\DrawEq[12]{p12 x1+x2}{12}
является следствием равенств
\eqRef{p(x)=(x-x1)(x-x2)}{12},
\EqRef{x=x1+x2}.
Равенство
\DrawEq[21]{p12 x1+x2}{21}
является следствием равенств
\eqRef{p(x)=(x-x1)(x-x2)}{21},
\EqRef{x=x1+x2}.
Утверждение
\EqRef{p12 ne p21}
является следствием равенств
\eqRef{p12 x1+x2}{12},
\eqRef{p12 x1+x2}{21}
и утверждения
\EqRef{x1x2/=x2x1}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{p=a1p12+a2p21}
Пусть
\ShowEq{a12 in AoxA}.
Тогда многочлен
\ShowEq{p=a1p12+a2p21}
имеет корни
\ShowEq{x=x1,x2}.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием утверждения,
что многочлены $p_{12}$, $p_{21}$
имеют корни
\ShowEq{x=x1,x2}.
\end{proof}

\begin{\QuestionStyle}
\labelQuestion{Does polynomial have other roots}
Имеет ли
многочлен
\EqRef{p=a1p12+a2p21}
корни отличные от значений
\ShowEq{x=x1,x2}?
\end{\QuestionStyle}

\begin{\QuestionStyle}
\labelQuestion{Are there other polynomials with given roots}
Существуют ли другие многочлены,
которые имеют корни
\ShowEq{x=x1,x2}?
\end{\QuestionStyle}

Похоже, что ответ на вопрос
\RefQuestion{Are there other polynomials with given roots}
положителен.

\begin{Example}
Рассмотрим множество многочленов
\ShowEq{p=a1 o ij+a2 o ji}
которые, согласно теореме
\RefTheorem{p=a1p12+a2p21},
имеют корни
\ShowEq{x=i,j}
Многочлен
\DrawEq{r=xx+1}{ij}
также имеет корни
\ShowEq{x=i,j}
\end{Example}

\begin{\QuestionStyle}
\labelQuestion{Does polynomial belong to the set of polynomials}
Принадлежит ли многочлен
\eqRef{r=xx+1}{ij}
множеству многочленов
\EqRef{p=a1 o ij+a2 o ji}?
\end{\QuestionStyle}

Теорема
\RefTheorem{a1 o ij+a2 o ji=xx+1}
отвечает на вопрос
\RefQuestion{Does polynomial belong to the set of polynomials}.

\begin{\TheoremStyle}
\labelTheorem{a1 o ij+a2 o ji=xx+1}
Не существует тензоров
\ShowEq{a12 in AoxA}{}
таких, что
\ShowEq{a1 o ij+a2 o ji=xx+1}
\end{\TheoremStyle}

\begin{proof}
Предположим, что теорема не верна.

\begin{Statement}
\labelStatement{there exist a12 in AoxA}
Пусть существуют тензоры
\ShowEq{a12 in AoxA}{}
таких, что
равенство
\EqRef{a1 o ij+a2 o ji=xx+1}
верно.
\hfill\(\odot\)
\end{Statement}

Равенства
\ShowEq{a1 o+a2 o=xx+1 xx}
\ShowEq{a1 o+a2 o=xx+1 x}
\ShowEq{a1 o+a2 o=xx+1 1}
следуют из равенства
\EqRef{a1 o ij+a2 o ji=xx+1}.

Пусть $x=1$.
Равенство
\ShowEq{a1 o+a2 o=xx+1 x x=1}
следуют из равенств
\EqRef{a1 o+a2 o=xx+1 x}.

Согласно теореме
\RefTheorem{sqrt a=...1+a},
существует $x$ такой, что $x^2=i$.
Равенство
\DrawEq[i]{a1 o+a2 o=xx+1 (ij) x x2=}i
следует из равенства
\EqRef{a1 o+a2 o=xx+1 xx}.

Согласно теореме
\RefTheorem{sqrt a=...1+a},
существует $x$ такой, что $x^2=j$.
Равенство
\DrawEq[j]{a1 o+a2 o=xx+1 (ij) x x2=}j
следует из равенства
\EqRef{a1 o+a2 o=xx+1 xx}.

Равенство
\ShowEq{a1 o+a2 o=xx+1 x x=1 1}
следует из равенств
\eqRef{a1 o+a2 o=xx+1 (ij) x x2=}i,
\eqRef{a1 o+a2 o=xx+1 (ij) x x2=}j
и противоречит равенству
\EqRef{a1 o+a2 o=xx+1 x x=1}.
Следовательно, утверждение
\RefStatement{there exist a12 in AoxA}
не верно и теорема доказана.
\end{proof}

\section{Деление с остатком}

\begin{\DefinitionStyle}
\labelDefinition{left divisor}
\(A\)\Hyph число \(a\)
называется левым делителем
\(A\)\Hyph числа \(b\),
если существует \(A\)\Hyph число \(c\)
такое, что
\ShowEq{ac=b}
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{right divisor}
\(A\)\Hyph число \(a\)
называется правым делителем
\(A\)\Hyph числа \(b\),
если существует \(A\)\Hyph число \(c\)
такое, что
\DrawEq{ca=b}{def}
\end{\DefinitionStyle}

Симметрия между определениями
\RefDefinition{left divisor}
и
\RefDefinition{right divisor}
очевидна.
Также как очевидно различие
между левым и правым делителями
в связи с некоммутативностью произведения.
Однако мы можем рассмотреть определение,
обобщающее определения
\RefDefinition{left divisor}
и
\RefDefinition{right divisor}.

\begin{\DefinitionStyle}
\labelDefinition{divisor of A number}
\(A\)\Hyph число \(a\)
называется делителем
\(A\)\Hyph числа \(b\),
если существует
\BoxB{A}число \(c\)
такое, что
\DrawEq[c]{c*a=b}{c}
\BoxB{A}число \(c\) называется
\AddIndex{частным от деления}{quotient divided by}
\(A\)\Hyph числа \(b\) на \(A\)\Hyph число \(a\).
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Пусть деление в \(D\)\Hyph алгебре \(A\)
не всегда определено.
\AddIndex{\(A\)\Hyph число $a$ делит \(A\)\Hyph число $b$ с остатком}
{division with remainder},
если следующее равенство верно
\DrawEq{c*a+f=b}{definition}
\BoxB{A}число \(c\) называется
\AddIndex{частным от деления}{quotient divided by}
\(A\)\Hyph числа \(b\) на \(A\)\Hyph число \(a\).
\(A\)\Hyph число $d$ называется
\AddIndex{остатком от деления}{remainder of the division}
\(A\)\Hyph числа \(b\) на \(A\)\Hyph число \(a\).
\end{\DefinitionStyle}

%\ShowTheorem{r=+q circ p}
%\ProofTheorem{1302.7204}{r=+q circ p}
\begin{\TheoremStyle}
\labelTheorem{r=+q circ (x-a)}
Пусть
\ShowEq{p=x-i}a
- многочлен степени $1$.
Пусть
\ShowEq{r power k}
многочлен степени $k>0$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{rk=rk0 ox rkk}
Согласно теореме
\RefTheorem{monomial of power k},
\ShowEq{rk xk=...}
Положим
\ShowEq{qk-1 xk-1=...}
Для доказательства теоремы
достаточно обратить внимание, что степень многочлена
\ShowEq{sk-1=r-qk-1 p}
меньше $k$.
Равенство
\ShowEq{r=sk-1+qk-1 p}
является следствием равенства
\EqRef{sk-1=r-qk-1 p}.
Мы применим рассуждения доказательства к многочлену $s_{k-1}(x)$.
После конечного числа шагов мы получим многочлен $s_0$ степени $0$.
Равенство
\EqRef{r=+q circ p}
является следствием равенства
\EqRef{r=sk-1+qk-1 p}.
\end{proof}

Алгоритм, рассмотренный в доказательстве теоремы
называется стандартный алгоритм деления многочленов.

\section{Примеры деления многочленов}

В последующих примерах мы применим стандартный алгоритм деления многочленов.

\ShowExample{r=x2-jx-xi-k p=x-i}

\ShowRemark{r=x2-jx-xi-k p=x-i}

\ShowRemark{r=x2-ix-xj+k p=x-i}

\ShowRemark{r=x2-ix-jx-k}

\ShowQuestion{r=x2-ix-jx-k}

\ShowRemark{r=x2-ix-jx-k 1}

\ShowRemark{r=x2-ix-jx-k p=x-j}

\ShowExample{r=x2-ix-jx-k p=x-j}

\section{Новые вопросы}

\ShowRemark{r=(x-j)(x-k)(x-j-k)}

\ShowQuestion{how to select factor in the tensor}

\ShowExample{select factor in the tensor}

\ShowRemark{select factor in the tensor}

\ShowExample{factorization as bilinear map}

\ShowQuestion{factorization as bilinear map}

Если многочлен $p(x)$ имеет вид
\ShowEq{p=p circ x}
где $p_1$ - невырожденный тензор,
то деление на многочлен $p(x)$
можно свести к теореме
\RefTheorem{r=+q circ (x-a)},
если мы воспользуемся равенством
\ShowEq{p=p1 (x+p1- p_0)}

\begin{\QuestionStyle}
Многочлен
\DrawEq[1]{ix-xi-1}{q1}
является делителем многочлена
\ShowEq{(x-j)(ix-xi-1)(x-k)}
Однако мы не можем воспользоваться теоремой
\RefTheorem{r=+q circ (x-a)}
для нахождения частного,
так как тензор
\ShowEq{1 ox i-i ox 1}
вырожден.
Поэтому необходимо дополнительное исследование,
чтобы решить эту задачу.
\end{\QuestionStyle}

\section{Деление многочленов в неассоциативной алгебре}

\begin{Remark}
В неассоциативной алгебре
скобки определяют в каком порядке мы выполняем умножение.
Поэтому одночлен может иметь следующий вид
\ShowEq{monomial (pq)r}
\ShowEq{monomial p(qr)}
где $p$, $q$, $r$ также одночлены.
Это накладывает ограничение
на возможность деления многочленов.
\end{Remark}

В примере
\RefExample{r=(x-j)(x-k)(x-jl)}
я рассмотрел многочлен $r(x)$ степени $3$
в алгебре октонионов.
Так как порядок множителей в произведении важен для определения структуры тензора,
я буду явно указывать скобки даже в тех случаях, когда порядок очевиден.
Например, поскольку, вообще говоря,
\ShowEq{((a ox)b)x ne (a (ox b))x}
то выражения
\ShowEq{(a ox)b}
и
\ShowEq{a (ox b)}
описывают различные линейные отображения.

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-jl)}
Пусть
\ShowEq{p=x-i}k
\DrawEq{r=(x-j)(x-k)(x-jl)}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q2=x2 (ox 1)}
Тогда
\ShowEq{s2=r-.p. 6}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=... 6}
Равенство
\ShowEq{s1=s2-.p. 6}
является следствием равенств
\EqRef{s2=r-.p. 6},
\EqRef{q1=... 6}.
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q0=... 6}
Равенство
\ShowEq{s0=s1-.p. 6}
является следствием равенств
\EqRef{s1=s2-.p. 6},
\EqRef{q0=... 6}.
Равенство
\ShowEq{r=s0+q1+q2 6}
является следствием равенств
\EqRef{s2=r-.p. 6},
\EqRef{q1=... 6},
\EqRef{q0=... 6},
\EqRef{s0=s1-.p. 6}.
\end{\ExampleStyle}

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-jl) x-j}
Частное от деления многочлена
\eqRef{r=(x-j)(x-k)(x-jl)}1
на многочлен
\ShowEq{p=x-i}k
имеет вид
\ShowEq{q(x)=  6}

\eqRef{r=(x-j)(x-k)(x-jl)}1
\FrameEq{r=(x-j)(x-k)(x-jl) 0}

Первое слагаемое тензора $q(x)$
имеет множитель $x-j$.
Чтобы проверить, имеет ли второе слагаемое
множитель $x-j$,
рассмотрим многочлен
\ShowEq{x^2-jx-xk+i}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x (ox 1)}
Тогда
\ShowEq{s1=r-.p. 8}
Теперь мы положим
\ShowEq{q0= 8}
Тогда
\ShowEq{s0=s-.p. 8}
Равенство
\ShowEq{r1=x2-jx-xk+i 8}
является следствием равенств
\EqRef{s1=r-.p. 8},
\EqRef{s0=s-.p. 8}.
\end{\ExampleStyle}

Из равенств
\EqRef{q(x)=  6},
\EqRef{r1=x2-jx-xk+i 8}
следует, что частное от деления многочлена
\eqRef{r=(x-j)(x-k)(x-jl)}1
на многочлен
\ShowEq{p=x-i}k
имеет вид
\ShowEq{r=(x-j)(x-k)(x-jl) q=}

\eqRef{r=(x-j)(x-k)(x-jl)}1
\FrameEq{r=(x-j)(x-k)(x-jl) 0}

Следовательно, мы можем представить многочлен
\eqRef{r=(x-j)(x-k)(x-jl)}1
в виде
\ShowEq{r=(x-j)(x-k)(x-jl) bilinear}

